Chance-Constrained Multi-Robot Motion Planning under Gaussian Uncertainties

We consider a chance-constrained multi-robot motion planning problem in the presence of Gaussian motion and sensor noise. Our proposed algorithm, CC-K-CBS, leverages the scalability of kinodynamic conflict-based search (K-CBS) in conjunction with the efficiency of the Gaussian belief trees used in the Belief-A framework, and inherits the completeness guarantees of Belief-A's low-level sampling-based planner. We also develop three different methods for robot-robot probabilistic collision checking, which trade off computation with accuracy. Our algorithm generates motion plans driving each robot from its initial state to its goal while accounting for the evolution of its uncertainty with chance-constrained safety guarantees. Benchmarks compare computation time to conservatism of the collision checkers, in addition to characterizing the performance of the planner as a whole. Results show that CC-K-CBS can scale up to 30 robots.

==> sections/collisionChecking.tex <==


\begin{figure}
    \centering
    \begin{subfigure}{0.26\textwidth}
    \includegraphics[width=\textwidth]{figures/minkVol.pdf}
    \vspace{-7mm}
    \caption{}
    \label{fig:CspaceIntegration}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.2\textwidth}
    \includegraphics[width=\textwidth]{figures/minkVolSlice.pdf}
    \vspace{-7mm}
    \caption{}
    \label{fig:CspaceIntegration_slice}
    \end{subfigure}
\caption{(a) 3D view of the c-space obstacle $\X_{coll}^{ij}$ 
% approximately constructed as the conjunction of a series of Minkowski sums of uncertain 
for
robot $i$ with fixed robot $j$ calculated at discrete choices of $\theta_k^i$.  
% (b) Example Minkowski sum for a single choice of $\theta_k^i$, depicted by the intersection of a gray plane in the top figure. 
(b)~Top-down view of $\X_{coll}^{ij}$.
The projection of $\X_{coll}^{ij}$ onto x-y plane is bounded by a green circle.}
\vspace{-3.5mm}
\end{figure}



Recall that the probability of collision between robots $i$ and $j$, as defined in  \eqref{eq:prob robot-robot collision}, requires integration of the joint probability distribution of the two robots over set $\X^{ij}_\coll$. 
The computation of this probability is difficult because (i) $\X^{ij}_\coll$ is hard to construct, and (ii) integration of the joint probability distribution function is expensive.  However, the constraint-checking procedure needs to be extremely fast in sampling-based algorithms because it is called in every iteration of the tree extension.  In this section, we introduce three approximation methods for this integration that trade off accuracy with computation effort.  
%The methods rely on bounding the projection of $\X^{ij}_{\coll}$ into the lower dimensional workspace, where checking the chance constraint is simpler. 

For clarity of explanation, consider two deterministic (rotating and translating) robots $i$ and $j$ in a 2D workspace, with configurations $(\text{x}_k^l,\text{y}_k^l,\theta_k^l)$, $l\in \{i,j\}$. We can construct the 4D c-space obstacles for this pair by taking the Minkowski difference of the two agents for every pair of orientation angles (see the c-space construction in Fig.~\ref{fig:CspaceIntegration}, which shows the c-space in 3D for a given orientation of agent $j$). This 4D obstacle is generally difficult to construct, so deterministic collision checkers typically resort to collision checking in the workspace, e.g., by bounding the projection of this set, shown by a green disk in Fig. \ref{fig:CspaceIntegration_slice}. 

Consider that each robot is described by a random variable (RV), so the position and orientation of their bodies are no longer deterministic but given by beliefs (distributions). This implies that each point in the 4D c-space has an associated probability. The exact probability of collision is the integral of the probability mass over the c-space obstacle. 
% Hence, the uncertain collision checking problem has two main challenges: construction of a complex c-space obstacle, and integration over this complex shape. 
This results in the two challenges listed above: c-space obstacle construction and integral computation.
Each method 
% listed in the following sections address these two core problems.
proposed below attempts to address these core problems. 
% Approximations and simplifications made to increase efficiency also introduce conservatism, which leads the collision checker to reject valid beliefs. Each of the methods described strikes a difference balance between these two competing factors.

%Then, the c-spaces are 3D and consist of a 2D Euclidean coordinate (position) and an orientation angle, i.e., $x_k^l=(\text{x}_k^l,\text{y}_k^l,\theta_k^l)$, $l\in \{i,j\}$. 
% These robots operate in a 2D workspace $\W$, so their projections $\proj{W}(x_k^l), l={i,j}$ are also 2D.
%Furthermore, assume only robot $i$ has uncertainty, and the state of robot $j$ is fixed and known. This reduces robot-robot collision checking to checking an uncertain robot with a known obstacle. In this case, the c-space is 3-dimensional, and the integration area for collision can be constructed by determining the Minkowski sum of the uncertain robot with the fixed robot for each possible orientation $\theta_k^i$. This is depicted by a pink volume in Figure \ref{fig:CspaceIntegration}. A simple way to bound the projection on $[\text{x}_k^i, \text{y}_k^i]$ space is to bound both robots' bodies with a disk that accounts for all possible orientations. The projection is then bounded by a circle with radius equal to the sum of the radii of the two bounding disks, shown as a green circle in Figure \ref{fig:CspaceIntegration}. The concept of bounding the projection in 2D euclidean space intuitively extends to higher dimensional state spaces. 

%We present three methods for checking the robot-robot collision constraint. Each method is computationally cheap, but has varying levels of conservatism. The sources of conservatism arise from two main sources: bounds on the orientation of the robot body, and approximations introduced to ease evaluation of complex integrals. The results section presents an empirical study of conservatism and computation time for various systems and environments. We present the methods in order of increasing computation time, and decreasing conservatism.
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/discBody.pdf}
         \vspace{-5mm}
         \caption{}
         \label{fig:diskBoundBody}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/individualAgentsProb.pdf}
         \vspace{-5mm}
         \caption{}
         \label{fig:AgentCircPsafe}
     \end{subfigure}
     \newline
     \begin{subfigure}[b]{0.45\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/DiskIntersect.pdf}
         \vspace{-5mm}
         \caption{}
         \label{fig:diskIntersect}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/diffProbCirc.pdf}
         \vspace{-5mm}
         \caption{}
         \label{fig:CircularBodyCicularIntegration}
     \end{subfigure}
     \newline
     \begin{subfigure}[b]{0.45\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/diffProbCircPoly.pdf}
         \vspace{-5mm}
         \caption{}
         \label{fig:CircularBodyPolygonIntegration}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/diffProbCircPoly_grid.pdf}
         \vspace{-5mm}
         \caption{}
         \label{fig:CircularBodyGridIntegration}
     \end{subfigure}
     \caption{
(a) Circle bound on robots' bodies. (b) $p_\safe$ contour and corresponding circular over bound on $p_\safe$. (c) Inflated circular bounds intersect, indicating possible collision between robots. (d) Integration area for probability of collision with circular disk bound on robots' bodies. (e) Polygonal bound on circular integration area. (f) Transformed distribution and integration area, with over-approximated grid.}
\vspace{-3.5mm}
\end{figure}

% \begin{figure}
%     \centering
%     \begin{subfigure}{0.3\textwidth}
%     \includegraphics[width=\textwidth]{figures/diffProbCirc.pdf}
%     \vspace{-7mm}
%     \caption{}
%     \label{fig:CircularBodyCicularIntegration}
%     \end{subfigure}
%     \\
%     \centering
%     \begin{subfigure}{0.3\textwidth}
%     \includegraphics[width=\textwidth]{figures/diffProbCircPoly.pdf}
%     \vspace{-7mm}
%     \caption{}
%     \label{fig:CircularBodyPolygonIntegration}
%     \end{subfigure}
% \caption{(a) Integration area for probability of collision with circular disk bound on robots' bodies. (b) Polygonal bound on circular integration area}
% \vspace{-3.5mm}
% \end{figure}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.3\textwidth]{figures/diffProbCircPoly_grid.pdf}
%     \vspace{-7mm}
%     \caption{}
%     \label{fig:CircularBodyGridIntegration}
% \caption{Transformed distribution and integration area, with over-approximated grid.}
% \vspace{-3.5mm}
% \end{figure}







\begin{comment}
%%% Old table, kept for reference for previous benchmarks    
\begin{table*}[]
    \centering
    \begin{tabular}{c|c|c|c|c}
         Method &  Body Bound & Integration Area & Bound on Integration Area & CC Evaluation\\
         \hline
         1 & Sphere & N/A & N/A & Intersection \\
         2 & Polyhedron & Polyhedron & N/A & Linear Constraint \\
         3 & Sphere & Sphere & Polyhedron & Linear Constraint \\
         4 & Sphere & Sphere & N/A & Grid CDF       
    \end{tabular}
    \caption{Summary table of collision checking methods.}
    \label{tab:ccMethodsSummary}
\end{table*}
\end{comment}

\subsection{Method 1: Safety Contour}
\label{sec:Method1}
Method 1 is inspired by deterministic collision checking methods, where collisions are detected by intersections of robot bodies in the workspace. We adapt this framework to uncertain collision checking by inflating bounds on the robot bodies to encapsulate $p_\safe$ probability mass.

%We rely on calculating a $w$-sphere for each robot in the workspace that is guaranteed to contain at least $p_{\safe}$ probability mass, we then check for collisions by ensuring these spheres do not intersect. A simplified 2D example is shown in Figures \ref{fig:diskBoundBody}, \ref{fig:AgentCircPsafe}, and \ref{fig:diskIntersect}.

Recall that the expected belief is $\expBelief(x_k^i)= \N(\check{x}_k^i,\Gamma_k^i)$. We define the Gaussian marginal of this distribution in the workspace as $\expBelief_\W(x_k^i)$.
% such that 
% \begin{equation}
%     \expBelief_\W(x_k^i) = \int_{\phi_k^i} \expBelief_{x_k^i\mid _k^i}(x_k^i\mid \phi_k^i)\expBelief_{\phi_k^i}(\phi_k^i)d\phi_k^i
% \end{equation}
Let $\bar{x}^i_k \in \W$ be the position components of $x_k^i$, and $\bar{\Gamma} \in \reals^{w\times w}$ be the corresponding covariance matrix (sub-matrix of $\Gamma^i_k$). Then $\expBelief_\W(x_k^i) = \N(\bar{x}^i_k, \bar{\Gamma}^i_k)$.
% \ml{hm.. why? Why don't we look at the belief of the projection of $x^i_k$ onto the workspace?  Let $\bar{x}^i_k \in \W$ be the position components of $x_k^i$, and $\bar{\Gamma} \in \reals^{w\times w}$ be the corresponding covariance matrix (sub-matrix of $\Gamma^i_k$). Then $\expBelief_\W(x_k^i) = \N(\bar{x}^i_k, \bar{\Gamma}^i_k)$, no? }
% where $\phi_k^i$ are all the state space variables not contained in the workspace. \at{Not so sure about this, is there a better way to write this?} 
The elliptical probability contour containing $p_{\safe}$ probability mass in the workspace marginal distribution is the region $\mathcal{E}_{\safe}^i$ such that
% \begin{equation*}
    $\int_{\mathcal{E}_{\safe}^i} \expBelief_\W(x_k^i) dx=p_{\safe}.$
% \end{equation*}
The axes of this ellipsoid are given by $a_l^i=t_{\chi}\lambda_l, \quad l=1,...,w,$ 
% $a^i_1,\ldots,a^i_w$ are defined by the eigenvalues of covariance $\bar{\Gamma}_k^i$
% , $eigenval(\Gamma_k^i)=(\lambda_1,...,\lambda_n)$, 
% such that 
% \begin{equation*}
%     a_l^i=t_{\chi}\lambda_l, \quad l=1,...,w,
% \end{equation*}
where $\lambda_l$ is an eigenvalue of $\bar{\Gamma}_k^i$, and
$t_{\chi}$ is the inverse $\chi^2$ cumulative density function
evaluated at $p_{\safe}$ with $w$ degrees of freedom.  

Determining intersection of ellipses is difficult, so we instead bound the ellipsoid with a sphere, where checking for intersection only requires comparing the sum of the radii to the distance between the centers. The sphere containing this ellipsoid, $\mathcal{C}_{\safe}^i$, is defined by the radius $r^i=t_{\chi}\lambda_{max}$, where 
% $\lambda_{max}=max(eigenval(\bar{\Gamma}_k^i))$. 
$\lambda_{\max}=\max\{ \lambda_l \}_{l=1}^w.$
Because $\mathcal{E}_{\safe}^i\subseteq \mathcal{C}_{\safe}^i$, it is assured that the probability mass contained by this sphere is greater than or equal to $p_{\safe}$, i.e., 
% \begin{equation}
    $\int_{\mathcal{C}_{\safe}^i} \expBelief_\W(x_k^i) dx\geq p_{\safe}.$
% \end{equation}
An illustration of both the elliptical contour and its associated spherical bound are shown in Fig.~\ref{fig:AgentCircPsafe} for the robots in Fig~\ref{fig:diskBoundBody}.

Note that this sphere contains only the probability mass associated with $x_k^i$, the origin point on the body frame. It does not account for the probability of any point on the body being in collision. To address this, we inflate this sphere by a bounding sphere on the robots body (shown in Fig.~\ref{fig:diskBoundBody}), such that the probability of \emph{any} point on the robot's body being within this inflated sphere is greater than or equal to $p_{\safe}$. The radius, $R_i$, of the bounding sphere on the robots body can be obtained by finding the largest possible Euclidean distance between any pair of points within a robot's body: $R_i = \frac{1}{2}\max_{x_1,x_2\in \B^i} \| x_1-x_2 \|_2$. The inflated bound, $\mathcal{C}_{bound}^i$ is then a sphere of radius $r^i+R^i$. The probability that any point of the robot is outside this sphere, the complement of $\mathcal{C}_{bound}^i$, is guaranteed to be less than $1-p_{\safe}$. Thus, if any two robot's bounding spheres
do not intersect, i.e. $\mathcal{C}_{bound}^i \cap \mathcal{C}_{bound}^j = \emptyset$, the probability of collision between them is guaranteed to be less than $1-p_{\safe}$.
% \begin{multline}
%     \mathcal{C}_{bound}^i \cap \mathcal{C}_{bound}^j = \emptyset  \quad \Rightarrow\\
%      P(\proj{\W}(x_k^i)) \cap \proj{\W}(x_k^j))\leq 1-p_{\safe}.
% \end{multline}
The inflated disks and corresponding intersection checking are shown in Fig.~\ref{fig:diskIntersect}.


%First, we bound the projection of all possible orientations of each robot in the workspace with a $w$-dimensional sphere ($w$-sphere), $S_{body}^i$. The bounding $w$-sphere is defined by radius $r^i$, see Figure \ref{fig:diskBoundBody}. Recall the state $x_k^i$ corresponds to the origin point of the body frame, we define this as the center of the sphere, with corresponding body frame coordinates $\text{w}^i$. We can define the body of the robot in its local frame as a set of $N_V^i$ vertices ${\text{v}_1^i,...,\text{v}_{N_V}^i}$. The radius $r_i$ can then be defined as the maximum radial distance between the origin point and the body vertices:
%\begin{equation}
%    r_i = \max_{\text{v}_l^i} \| \text{w}^i - \text{v}_l^i\|_2, \quad l=1,...,N_V^i
%\end{equation}
%\at{added stuff about the vertices of the body, but I'm not sure how to formally define these...Should probably be up in the problem formulation section too}

%We use this bounding sphere to inflate the probability set calculated in the following paragraph, extending the constraint from the point distribution to cover the full body of the robot.


%Note that this sphere contains only the probability mass associated with $x_k^i$, the origin point on the body frame, it does not account for the probability of any point on the body being in collision. To address this, we inflate this sphere by the bounding sphere, such that the probability of \emph{any} point on the robot's body being within this new bounding sphere is assured to be greater than or equal to $p_{\safe}$. We denote this new bounding sphere by $\mathcal{C}_{bound}^i$, with radius $r^i+R^i$. This inflated bound is depicted in Figure \ref{fig:diskIntersect}. The probability that any point of the robot is outside this circle, the complement of $\mathcal{C}_{bound}^i$, is guaranteed to be less than $1-p_{\safe}$. Thus, if any two robot's bounding circles do not intersect, the probability of collision between them is guaranteed to be less than $1-p_{\safe}$:
%\begin{multline}
%    \mathcal{C}_{bound}^i \cap \mathcal{C}_{bound}^j = \emptyset  \quad \Rightarrow\\
%     P(\proj{\W}(x_k^i)) \cap \proj{\W}(x_k^j))\leq 1-p_{\safe}.
%\end{multline}

This method has two main sources of conservatism. The first stems from the bounding sphere on the robot body. This is especially egregious for robots with high aspect ratios. The second source is associated with checking for intersections of the probability mass bound. This conservatively assumes all probability mass not within the sphere is in collision, so any intersection (no matter how small) is considered a possible constraint violation. Violation for this method does not imply that the actual probability of collision exceeds the constraint. Despite these limitations, this method is extremely fast. %collision checking method.
% of all those proposed here.

\subsection{Method 2: Linear Gaussian Transformation}
\label{sec:Method2}
This section introduces a class of methods that reduce conservatism by simplifying the integration itself, namely by reducing its dimensionality. This is done by introducing a new RV representing the difference between two robots' states: $x_k^{ij}=x_k^i-x_k^j$. This RV is Gaussian distributed such that $x_k^{ij}\sim\N(\check{x}_k^i-\check{x}_k^j, \Gamma_k^i+\Gamma_k^j)$, with the workspace marginal $\expBelief_\W(x_k^{ij})$. This new RV represents a vector connecting the origin points of two robots. Collisions correspond to specific realizations of $x_k^{ij}$, %this difference vector, 
defining the required integration  area. 

\begin{comment}
\begin{figure}
    \centering
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/polyBodyBound.pdf}
    \vspace{-7mm}
    \caption{}
    \label{fig:polyBodyBound}
    \end{subfigure}
    \centering
    \begin{subfigure}{0.3\textwidth}
    \includegraphics[width=\textwidth]{figures/diffProbMinkPoly.pdf}
    \vspace{-7mm}
    \caption{}
    \label{fig:PolyBodyMinkowskiInt}
    \end{subfigure}
\caption{(a) Integration area for probability of collision with circular disk bound on robots' bodies. (b) Polygonal bound on circular integration area}
\vspace{-3.5mm}
\end{figure}


\subsubsection{ditching this method}
This method relies on a polyhedral bounds on the bodies of the robots in the workspace, these bounds are then used to construct Minkowski sums which define the integration area. Because this is still a complex integration area, we simplify the constraint checking by using the approximate linear constraints first derived for CC-RRT in \cite{Luders2010_CC-RRT}.

For each robot we define a polyhedra in the workspace, $\mathcal{P}_{poly}^i$,  that bounds the robot's body for all possible orientations. This can be constructed by defining a polyhedral bound over the sphere $S_{body}^i$ described in Section \ref{sec:Method1}, shown in Figure \ref{fig:polyBodyBound}. \at{Need more explanation here?}. We construct the Minkowski Sum for all possible pairs of robots, $\mathcal{P}_{Mink}^{ij}$. 

We then introduce a new random variable, $x_k^{ij}=x_k^i-x_k^j$ representing the difference between two robots' states, this random variable is Gaussian distributed such that $x_k^{ij}\sim\N(\check{x}_k^i-\check{x}_k^j, \Gamma_k^i+\Gamma_k^j)$, with the workspace marginal $\expBelief_\W(x_k^{ij})$. By integrating $\expBelief_\W(x_k^{ij})$ over the Minkowski sum, we can exactly find the probability of the two bounding polyhedra intersecting (indicating possible collision), shown in Figure \ref{fig:PolyBodyMinkowskiInt}. To check the chance constraint, we simply need to ensure this probability does not exceed $1-p_{\safe}$. However, this integral is difficult to calculate, so further approximation is required. We instead make the following approximations to simplify checking the chance constraint. 

The Minkowski sum can be given by the conjunction of a set of $N_p$ half planes: $\mathcal{P}_{Mink}^{ij} = \{ x \mid \mathrm{a}_{h,i}^Tx<b_{h,i}, \forall h\in[1,N_p]\}$, where $a_{h,i}\in\mathbb{R}^{1\times w}$ and $b_{h,i}\in\mathbb{R}$. This reduces the robot-robot chance constraint checking problem to the same problem addressed in \cite{Luders2010_CC-RRT}. In that work, various approximations were used to reduce the probabilistic chance constraint checking problem to checking a set of deterministic linear constraints. One of the key approximations was the allocation of the acceptable probability of collision, or risk allocation: the total acceptable probability of collision ($\Delta = 1-p_{\safe}$) must be distributed across all the possible sources of collision. In our case, we must distribute the probability of collision for an robot among the $N_A-1$ other robots. To keep things general, we we will denote the allowable probability for robot $i$ colliding with any other robot $j$ as $p_c^{ij}$. Two proposed methods of determining $p_c^{ij}$ are described in Section \ref{sec:Risk Allocation}. Under this generalization, we have adapted the linear constraints from \cite{Luders2010_CC-RRT} for the random variable $x_k^{ij}$ as:
\begin{multline}
    \bigvee_{h=1}^{N_p} a_{h,i}^T (\check{x}_k^i-\check{x}_k^j) \geq b_{h,i} + \bar{b}_{h,i}  \quad \Rightarrow  \\
    P(\proj{\W}(X_k^i)) \cap \proj{\W}(X_k^j))\leq 1-p_{\safe}
\end{multline}
where
\begin{align}    
    &\bar{b}_{h,i} = \sqrt{2}P_v erf^{-1}\left( 1-2 p_c^{ij} \right), \\
    &P_v = \sqrt{a_{h,i}^T(\Gamma_k^i+\Gamma_k^j)a_{h,i}}
\end{align}

There are two main sources of conservatism here. The first stems from the same source as the prior method: the polyhedral bound on the body is even more conservative than the spherical bound. This results in violation of the constraint in cases where the true orientations of the body do not actually intersect. The second source of conservatism arises from the use of deterministic linear constraints for the integration itself. This source of conservatism scales with the number of robots and the number of half planes in the Minkowski sum. This method is only slightly more computationally intensive than the first method. While checking linear constraints is very computationally simple, this method must at worst check every constraint for associated with each pair of robots. This yields slightly longer computation times than the first method, which required checking a single condition for every robot pair.
\end{comment}



\subsubsection{Method 2.1: Convex Polytopic Bounding}
\label{sec:Method2.1}
%Note that 
The difference RV somewhat simplifies the high dimensional c-space obstacle representation, shown in Fig.~\ref{fig:CspaceIntegration}, by merging the workspace dimensions for the two robots. But the orientation of the robots still must be considered. To obtain a tractable integration area, we use the same bounding spheres described in Sec.~\ref{sec:Method1}. Intersection of the bounding spheres is considered a collision state, corresponding to a spherical integration area $S_{body}^{ij}$, with radius $R^i + R^j$, over difference distribution $\expBelief_\W(x_k^{ij})$ (shown in Fig.~\ref{fig:CircularBodyCicularIntegration}). 

Because exact integration of a Gaussian distribution over a sphere is difficult, we bound $S_{body}^{ij}$ with a polytope, $\mathcal{P}_{body}^{ij}$, which can be defined by a set of $N_s$ half planes, $\mathcal{P}_{body}^{ij} = \{ x \mid c_{h,i}^Tx<d_{h,i}, \forall h\in[1,N_s]\}$, where $c_{h,i}\in\mathbb{R}^{n\times 1}$ and $d_{h,i}\in\mathbb{R}$. This reduces the robot-robot chance constraint checking problem to the same problem addressed in \cite{Luders2010_CC-RRT},  where various approximations are used to reduce the probabilistic chance constraint checking to deterministic linear constraints checking. We employ those same methods to check the chance constraints, with the distribution given by $\N(\check{x}_k^i-\check{x}_k^j, \Gamma_k^i+\Gamma_k^j)$, and polytope given by $\mathcal{P}_{body}^{ij}$.

A key approximation in this method is the allocation of the acceptable probability of collision, or risk allocation: the total acceptable probability of collision $p_{coll} = 1-p_{\safe}$ must be distributed across all the possible sources of collision. In our case, we must distribute the probability of collision for a robot among the $N_A-1$ other robots. We denote the allowable probability for robot $i$ colliding with any other robot $j$ as $p_c^{ij}$. Two proposed methods of determining $p_c^{ij}$ are described in Sec.~\ref{sec:Risk Allocation}. 
% Under this generalization, we have adapted the linear constraints from \cite{Luders2010_CC-RRT} for the random variable $x_k^{ij}$ as:
% \begin{multline}
%     \text{if} \quad \bigvee_{h=1}^{N_c} c_{h,i}^T (\check{x}_k^i-\check{x}_k^j) \geq d_{h,i} + \bar{d}_{h,i} \\
%     \rightarrow P(\proj{\W}(X_k^i)) \cap \proj{\W}(X_k^j))\leq 1-p_{\safe}
% \end{multline}
% where 
% \begin{multline}    
%     \bar{d}_{h,i} = \sqrt{2}P_v erf^{-1}\left( 1-2 p_c^{ij} \right), \\
%     P_v = \sqrt{c_{h,i}^T(\Gamma_k^i+\Gamma_k^j)c_{h,i}}
% \end{multline}

This method has two main sources of conservatism. The first source is associated with the spherical bound on the body, the same as in Sec.~\ref{sec:Method1}. The second source of conservatism arises from the use of deterministic linear constraints for the integration itself. This source of conservatism scales with the number of robots and the number of half planes in the polytope bound. This method is only slightly more computationally intensive than the first method: while checking linear constraints is very computationally simple, this method must at worst check every constraint for associated with each pair of robots. This yields slightly longer computation times than the first method, which requirs checking a single condition for every robot pair. 


\subsubsection{Method 2.2: Grid Integration}
This method follows directly from Method 2.1, but with a direct integration technique, rather than a check on deterministic linear constraints. This makes this method more accurate and less conservative, but also more computationally intensive. 

We begin with the same difference distribution over $\expBelief_\W(x_k^{ij})$ 
and integration over $\mathcal{P}_{body}^{ij}$. We then perform a whitening (Mahalanobis) transformation on the distribution and $\mathcal{P}_{body}^{ij}$. This transformation decorrelates a Gaussian distribution, yielding the standard normal distribution, as well as rotating and translating $\mathcal{P}_{body}^{ij}$. We define this new integration area as $\mathcal{P}_{white}^{ij}$ (see Fig.~\ref{fig:CircularBodyGridIntegration}). 
Because we have transformed the probability distribution to a standard normal, the cumulative distribution function can be easily computed via the error function (erf); we do this over a grid. This technique is agnostic to the choice of grid cells and only requires rectangular cells that completely cover the polytope $\mathcal{P}_{white}^{ij}$, as shown in green in Fig. \ref{fig:CircularBodyGridIntegration}. The probability of collision is the sum of the probability mass contained in each grid cell, defined as $p_{poly}$. The chance constraint can then be simply checked as $p_{poly}\leq 1-p_\safe$.

%we will define a grid discretization over the entire workspace, with discretization step size for each workspace axis as $d\W_w$.  Each grid cell, $\W_g$, is a defined as set of vertices, $v_\W\in\W$, such that the $w$-th element of $v_\W$, $v_{\W}(w)$ is an element of the adjacent set of grid points in axis $w$:
%\begin{equation}
%    v_{\W}(w) \in \{w_Nd\W_w, (w_N+1)d\W_w\}, \quad w_N\in\mathbb{Z}
%\end{equation}
%The set of cells that over-approximate the integration area is therefore: $\W_{g,poly}=(\W_g \mid \exists v_\W(w) \in \mathcal{P}_{whit}^{ij})$. This grid over approximation of the integration area is shown in Figure \ref{fig:CircularBodyGridIntegration}.
%\at{Bonkers way to define a grid, there must be a better way...}

%The probability contained in a grid cell, $p(\W_g)$ can then be defined in terms of the cdf evaluated at each vertex:
%\begin{equation}
%    cdf(v_\W) = \prod_{w} \frac{1}{2}\left( 1 + erf\left( \frac{v_\W(w)}{\sqrt{2}} \right) \right)
%\end{equation}

%The over approximation of the probability mass contained in $\mathcal{P}_{whit}^{ij}$, defined as $p_{poly}$ is 
%\begin{equation}
%    p_{poly} = \sum_{\W_g\in\W_{g,poly}} p(\W_g)
%\end{equation}

% The chance constraint can then be simply checked as:
% \begin{multline}
%     \text{if} \quad p_{poly}\leq p_\safe \\
%     \rightarrow P(\proj{\W}(X_k^i)) \cap \proj{\W}(X_k^j))\leq 1-p_{\safe}
% \end{multline}
This method inherits the same conservatism associated with the spherical body bound and polytope integration area bound in Method 2.1. However, the approximate grid probability calculation is far less conservative than the deterministic linear constraints. The grid introduces more computational complexity, particularly in transforming the distribution and evaluating the probability of each grid cell. Finer grid discretization reduces conservatism, but also increases computation time.

\subsection{Risk Allocation}
\label{sec:Risk Allocation}
%Note that 
Risk allocation is only necessary for Methods 2 and not required in Method 1. Equally distributing the allowable probability of collision $p_{coll}$ across the robots and obstacles, as introduced in \cite{Luders2010_CC-RRT}, is the simplest allocation method. For robot-robot collision this corresponds to $p_c^{ij}=\frac{p_{coll}}{N_O + N_A - 1}$. However, this can be overly conservative and make it difficult to find viable motion plans. Instead, we propose allocating $p_{coll}$ more effectively, such that robots with a higher likelihood of collision are assigned a higher proportion of $p_{coll}$.

We begin by setting $p_{coll}=P_c^A+P_c^O$, where $P_c^A$ 
% is the allowable probability of collision with all the robots, and 
and
$P_c^O$ are the allowable probabilities of collision with all the robots and all the static obstacles, respectively. This naturally fits the high-level low-level division in CC-K-CBS because obstacle collision checking occurs only in the low-level planner.
Define the total volume of all the robots as $V_A$, and the volume of all the obstacles as $V_O$. Then, we set  $P_c^A=\frac{V_A p_{coll}}{V_A+V_O}$ and $P_c^O=\frac{V_Op_{coll}}{V_A+V_O}$. This allocates more of the probability of collision to the category that is more likely to cause collisions. 
We then divide $P_c^A$ based on the distance between robots, with robots that are closer together receiving a larger portion of $P_c^A$. Let $d_k^{j}=\|\bar{x}_k^i-\bar{x}_k^j\|$ be the workspace distance between robot $i$'s and $j$'s means. Then, the allowable probability of collision for robot $i$ with $j$ is $p_c^{ij} = \frac{\alpha}{d_k^j}P_c^A$, where 
% $\alpha =\frac{1}{\sum_j^{N_A-1} d_k^{j}}$ 
$\alpha =1/ (\sum_j^{N_A-1} d_k^{j})$ 
is the normalizing factor.


==> sections/conclusion.tex <==
We consider the MRMP problem under Gaussian uncertainty. We propose an algorithm, CC-K-CBS, which generates motion plans for each robot while providing guarantees on satisfying chance constraints on the probability of collision with obstacles and other robots. This algorithm is based on extending K-CBS to accommodate belief space planning using belief-$\mathcal{A}$. Our main contribution is 3 different methods for checking for collisions between probabilistic robots. We provide benchmarks comparing the computation time and conservatism of each proposed method, as well as benchmarks characterizing the performance of CC-K-CBS as a whole. This first attempt at uncertain MRMP method successfully generated motion plans across a variety of scenarios and scaled to 25 robots in an empty environment, however further work could encompass other types of noise and nonlinear dynamics. Additionally, new collision methods could further improve computation time and conservatism.

==> sections/evaluation.tex <==

% We implemented CC-K-CBS with belief-SST as the low-lever planner in Open Motion Planning Library (OMPL), 
% The benchmarks were performed on AMD Ryzen 9 4.5GHz CPU and 64 GB of RAM.
We evaluate our algorithms in several benchmarks. We first focus on characterizing the robot-robot collision checking algorithms from Sec.~\ref{sec:collisionChecking} independent of the planning algorithm. This allows us to isolate the conservatism and computational complexity of the robot-robot collision checkers. We then analyze the full algorithms from Sec.~\ref{sec:method} with different collision checking methods
Our implementation of CC-K-CBS uses belief-SST as the low-lever planner in Open Motion Planning Library (OMPL), 
the benchmarks were performed on AMD 4.5 GHz CPU and 64 GB of RAM. 
% this allows us to examine how the larger planning framework behaves as whole, and better evaluate the situations where one collision checker is advantageous over the other.

\begin{figure}
    \centering
    \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/conservatism.pdf}
    \vspace{-7mm}
    \caption{}
    \label{fig:conservatism}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/CompTime_combined.pdf}
    \vspace{-7mm}
    \caption{}
    \label{fig:compTime_combined}
    \end{subfigure}
    \hfill

\caption{(a) Plot of the conservatism $C_{z}$ for each method in each environment. (b) Box and whiskers plots of the log(computation time) for each method.}
\vspace{-3.5mm}
\end{figure}

We consider two types of robot dynamics and varying number of robots $N_A$. The first is a 2D system taken from~\cite{Bry2011_BeliefProp}:
% \begin{align}
    $x_{k+1}^i=x_k^i+u_k^i+w_k^i$ with $w_k^i \sim \mathcal{N}(0,0.1^2I)$.
% \end{align}
The second is a second-order unicycle:
% \begin{equation}
    % \dot{\text{x}}^i= \text{v} \cos\theta, \quad \dot{\text{y}}^i= \text{v} \sin \theta, \quad \dot{\theta}=\omega, \quad \dot{\text{v}}=a,
% \end{equation}
$\dot{\text{x}}^i= \text{v} \cos\theta,$ $\dot{\text{y}}^i= \text{v} \sin \theta$, $\dot{\theta}=\omega$, $\dot{\text{v}}=a$,
where $\omega$ and $a$ are control inputs. We use the feedback linearization scheme described in \cite{DeLuca2000_feedbackLin} to obtain a linear model, 
%with $x_k^i=[\text{x}_k^i,\dot{\text{x}}_k^i, \text{y}_k^i,\dot{\text{y}}_k^i]$ and noise $Q^i=0.1^2I$. 
which we convert to discrete time. We assume both systems are fully observable with measurement model~\eqref{eq: measurement model} with $C^i=I$ and $R^i=0.1^2I$.


% \subsection{Robot-Robot Collision Checker Benchmarking}
\textbf{Robot-Robot Collision Checker Benchmark: }
We characterize the robot-robot collision checking algorithms based on computation time and conservatism. Conservatism impacts the planners ability to find paths in more difficult, i.e. cluttered, situations. For a given set of beliefs for two robots, we define the conservatism of method $z$ as $C_{z} = R_{z} - R_{MC}$, where $R_{z}$ is the rejection rate obtained by method $z$, and $R_{MC}$ is the rejection rate obtained by a Monte Carlo evaluation of the probability of collision.

% from the \emph{true} probability of collision, $p_{true}^{ij}$. 

% If the true probability is know, the chance constraint can be exactly evaluated: $p_{true}^{ij}<1-p_\safe$. To evaluate conservatism, we randomly sampled $N_{MC}$ sets of two beliefs for each agent, $B_{s_{ij}}=\{\expBelief^i, \expBelief^j\}, s_{ij}=1,...,N_{MC}$, with $N_{MC}=10,000$. For each pair, we then computed the true probability of collision, and evaluated the chance constraint to obtain either valid or invalid, $\bar{v}^{s_{ij}}=1$ or $0$ respectively. The true validity rate can then be calculated as $\bar{V}_{true}=\sum_{s_{ij}=1}^{N_{MC}} \bar{v}^{s_{ij}}/N_{MC}$. For each pair, we then evaluate the chance constraint according to each of the proposed collision checking algorithm, $\bar{v}_{alg}^{s_{ij}}\in\{0,1\}$, yielding an associated algorithmic validity rate $\bar{V}_{alg}=\sum_{s_{ij}=1}^{N_{MC}} \bar{v}_{alg}^{s_{ij}}/N_{MC}$. Conservatism is defined as the difference between the true validity rate and the algorithmic validity rate: $C_{alg}=\bar{V}_{alg}-\bar{V}_{true}$. This indicates how often the algorithm rejects as invalid a sample that actually satisfies the chance constraint.


% \ml{all you're saying is that conservatism of method $z$ is defined as $C_{z} = R_{z} - R_{MC}$, where $R_{z}$ is the rejection rate obtained by method $z$, and $R_{MC}$ the rejection rate obtained by Monte Carlo evaluation of the probability of collision????}

% \ml{is this paragraph needed?}
% As stated earlier, the entire motivation for the proposed agent-agent collision checking algorithms is the difficulty of evaluating the true probability of collision. For the benchmarks performed here, we approximate the true probability of collision via MC sampling. For each pair of sampled beliefs, we further sampled 50,000 states. Each sampled state corresponds to a projection of the robots bodies in the workspace, where collision is indicated by the intersection of the two projections. To calculate the 'true' probability of collision, we found the proportion of the sampled states that resulted in collision.

We sampled 2D beliefs in two difference spaces, 5x5 and 10x10, with $p_\safe=0.95$. For Method 2.2 (the gridded cdf method), we chose 6 different grid discretizations, denoted by Method 2.2($d$). For each discretization, the maximum range of $\mathcal{P}_{whit}^{ij}$ over each axis, $D_w$, was divided equally, such that the discretization step size was $D_w/d$. Note that each of the proposed methods decreases in conservatism, shown in Fig.~\ref{fig:conservatism}, and increases in computation time, shown in Fig.~\ref{fig:compTime_combined}. The 5x5 space is the more `cluttered', with more beliefs in close proximity, which in turn results in higher collision probabilities. Note that the 5x5 space generally results in lower conservatism. This is because for the relatively high choice of $p_\safe$, a high proportion of the sampled beliefs truly violated the chance constraint, making it less conservative compared to a scenario where more beliefs are valid.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/PcollVSdist_Comp.pdf}
%     \vspace{-2mm}
%     \caption{Plot of the true probability of collision vs the euclidean distance between the means for each sampled belief pair}
%     \label{fig:PcollvsDist}
%     \vspace{0mm}
% \end{figure}







% \begin{table}[]
% \caption{CC-K-CBS and Centralized planner benchmarking results for simple 2D linear system}
%     \centering
%     \scalebox{0.65}{
%     \begin{tabular}{|c|c|c|c|c|c|}
%          \hline
%             & \multicolumn{4}{c|}{Decentralized (CC-K-CBS)} & Centralized \\
%             & Method 2.2 & Method 2.1* & Method 2.1 & Method 1 & Method 1\\ \hline
%             \multirow{3}{*}{2 Agents}  &     1.00 &   1.00 &   1.00 &   1.00 & 1.00\\ 
%             & 1.26 $\pm$   1.41 &   1.56 $\pm$   1.91&   1.41 $\pm$   1.21&   1.36 $\pm$   1.03& N/A\\ 
%             & 93.72 $\pm$  13.18 &  94.73 $\pm$  14.34&  90.07 $\pm$  13.05&  91.76 $\pm$  12.87& 81.07 $\pm$  17.67\\    \hline
%            \multirow{3}{*}{3 Agents}  &  1.00 &   1.00 &   1.00 &   1.00 &   1.00\\ 
%               & 1.87 $\pm$   1.40 &   2.10 $\pm$   1.84&   2.25 $\pm$   1.32&   3.52 $\pm$   3.77& N/A \\ 
%             & 136.22 $\pm$  12.96 & 130.30 $\pm$  13.41& 133.11 $\pm$  15.35& 133.93 $\pm$  13.63 & 108.76 $\pm$  22.97 \\  \hline
%            \multirow{3}{*}{5 Agents}  &   1.00 &   1.00 &   1.00 &   1.00 & \\ 
%                 &  8.94 $\pm$   7.47 &  15.12 $\pm$  13.22&  13.70 $\pm$  12.06&  16.47 $\pm$  16.99& N/A\\ 
%                 & 167.17 $\pm$  15.65 & 167.34 $\pm$  14.74& 170.24 $\pm$  19.59& 177.61 $\pm$  19.62& N/A\\   \hline
%              \multirow{3}{*}{7 Agents} &   0.76 &   0.44 &   0.66 &   0.52 & \\ 
%                  & 62.75 $\pm$  52.59 &  76.51 $\pm$  38.41&  81.55 $\pm$  52.70&  67.57 $\pm$  45.73& N/A\\ 
%                 & 293.11 $\pm$  17.95 & 286.35 $\pm$  19.10& 281.48 $\pm$  17.85& 299.11 $\pm$  19.40& N/A\\  
%         \hline
        
%     \end{tabular}
%     }
%     \label{tab:benchCCKCBS_linear}
% \end{table}



\begin{table*}[t!]
\caption{CC-K-CBS benchmarking for Simple 2D and unicycle systems}
    \centering
    \scalebox{0.7}{
    \begin{tabular}{|c|c||c|c|c|c||c|c|c|c|}
         \hline
          & & \multicolumn{4}{c||}{Simple Linear} & \multicolumn{4}{c|}{Unicycle}  \\
         $\#$ Robots & Metric & Method 2.2 & Method 2.1* & Method 2.1 & Method 1& Method 2.2 & Method 2.1* & Method 2.1 & Method 1\\ \hline 
        \multirow{3}{*}{2} &  Succ. Rate &  1.00&   1.00 &   1.00 &   1.00 &  1.00&   1.00 &   1.00 &   1.00\\ 
         &  Time (s) &    1.36 $\pm$   0.15 &   1.36 $\pm$   0.19&   1.56 $\pm$   0.27&  \textbf{ 1.26 $\pm$   0.20}&    4.07 $\pm$   0.48 &  \textbf{ 2.77 } $\pm$   0.31&   4.79 $\pm$   0.74&   5.03 $\pm$   0.69\\ \hline 
        \multirow{3}{*}{3} &  Succ. Rate &  1.00&   1.00 &   1.00 &   1.00 &  1.00&   1.00 &   1.00 &   1.00\\ 
         &  Time (s) &    3.52 $\pm$   0.53 &   2.33 $\pm$   0.29&   2.10 $\pm$   0.26&  \textbf{ 1.87 $\pm$   0.20} &    6.18 $\pm$   0.63 &  \textbf{ 4.58 $\pm$   0.54}&  11.30 $\pm$   1.82&   7.36 $\pm$   1.32\\ \hline 
        \multirow{3}{*}{5} &  Succ. Rate &  1.00&   1.00 &   1.00 &   1.00 &  1.00&   1.00 &   1.00 &   1.00\\ 
         &  Time (s) &   16.47 $\pm$   2.40 &  11.89 $\pm$   2.00&  15.12 $\pm$   1.87&  \textbf{ 8.94 $\pm$   1.06} &   13.59 $\pm$   1.72 &  \textbf{ 7.34 $\pm$   1.05}&  21.73 $\pm$   2.70&  13.94 $\pm$   1.71\\ \hline 
        \multirow{3}{*}{7} &  Succ. Rate &  0.52&   0.66 &   0.44 &  \textbf{ 0.76} &  0.40&   0.50 &   0.24 &  \textbf{ 0.56}\\ 
         &  Time (s) &   67.57 $\pm$   8.97 &  62.99 $\pm$   6.81&  76.51 $\pm$   8.19& \textbf{ 62.75 $\pm$   8.53} &  \textbf{ 66.44 $\pm$   8.22 }& 100.77 $\pm$   8.37&  77.15 $\pm$  10.52&  82.92 $\pm$   7.51\\ \hline       
    \end{tabular}
    }
    `\vspace{-4mm}
    \label{tab:benchCCKCBS}
\end{table*}



% \begin{table}[]
% \caption{CC-K-CBS benchmarking for 2D system}
%     \centering
%     \scalebox{0.7}{
%     \begin{tabular}{|c|c|c|c|c|c|}
%          \hline
%          $\#$ Robots & Metric & Method 2.2 & Method 2.1* & Method 2.1 & Method 1\\ \hline 
%         \multirow{3}{*}{2 Robots} &  Succ. Rate &  1.00&   1.00 &   1.00 &   1.00\\ 
%          &  Time (s) &    1.36 $\pm$   0.15 &   1.36 $\pm$   0.19&   1.56 $\pm$   0.27&  \textbf{ 1.26 $\pm$   0.20}\\ \hline 
%         \multirow{3}{*}{3 Robots} &  Succ. Rate &  1.00&   1.00 &   1.00 &   1.00\\ 
%          &  Time (s) &    3.52 $\pm$   0.53 &   2.33 $\pm$   0.29&   2.10 $\pm$   0.26&  \textbf{ 1.87 $\pm$   0.20}\\ \hline 
%         \multirow{3}{*}{5 Robots} &  Succ. Rate &  1.00&   1.00 &   1.00 &   1.00\\ 
%          &  Time (s) &   16.47 $\pm$   2.40 &  11.89 $\pm$   2.00&  15.12 $\pm$   1.87&  \textbf{ 8.94 $\pm$   1.06}\\ \hline 
%         \multirow{3}{*}{7 Robots} &  Succ. Rate &  0.52&   0.66 &   0.44 &  \textbf{ 0.76}\\ 
%          &  Time (s) &   67.57 $\pm$   8.97 &  62.99 $\pm$   6.81&  76.51 $\pm$   8.19& \textbf{ 62.75 $\pm$   8.53}\\ \hline        
%     \end{tabular}
%     }
%     \label{tab:benchCCKCBS_linear}
% \end{table}
% \begin{table}[]
%     \centering
%     \caption{CC-K-CBS benchmarking for unicycle system}
%     \scalebox{0.7}{
%     \begin{tabular}{|c|c|c|c|c|c|}
%          \hline
%         $\#$ Robots & Metric & Method 2.2 & Method 2.1* & Method 2.1 & Method 1\\ \hline 
%         \multirow{3}{*}{2 Robots} &  Succ. Rate &  1.00&   1.00 &   1.00 &   1.00\\ 
%          &  Time (s) &    4.07 $\pm$   0.48 &  \textbf{ 2.77 } $\pm$   0.31&   4.79 $\pm$   0.74&   5.03 $\pm$   0.69\\ \hline 
%         \multirow{3}{*}{3 Robots} &  Succ. Rate &  1.00&   1.00 &   1.00 &   1.00\\ 
%          &  Time (s) &    6.18 $\pm$   0.63 &  \textbf{ 4.58 $\pm$   0.54}&  11.30 $\pm$   1.82&   7.36 $\pm$   1.32\\ \hline 
%         \multirow{3}{*}{5 Robots} &  Succ. Rate &  1.00&   1.00 &   1.00 &   1.00\\ 
%          &  Time (s) &   13.59 $\pm$   1.72 &  \textbf{ 7.34 $\pm$   1.05}&  21.73 $\pm$   2.70&  13.94 $\pm$   1.71\\ \hline 
%         \multirow{3}{*}{7 Robots} &  Succ. Rate &  0.40&   0.50 &   0.24 &  \textbf{ 0.56}\\ 
%          &  Time (s) &  \textbf{ 66.44 $\pm$   8.22 }& 100.77 $\pm$   8.37&  77.15 $\pm$  10.52&  82.92 $\pm$   7.51\\ \hline 
%     \end{tabular}
%     }
%     \label{tab:benchCCKCBS_unicycle}
% \end{table}


% \subsection{Characterizing the MRMP Planners}
\textbf{Characterizing the MRMP Planners: }
% We first compare benchmarks on the performance of the centralized and CC-K-CBS planners proposed in Sec.~\ref{sec:method}. We then present specific plans generated by the decentralized method, along with results from Monte Carlo (MC) simulations demonstrating the plans' validity. 
% \subsubsection{Planner Benchmarking}
We use benchmarking to compare the centralized planner to CC-K-CBS under each of the methods proposed in Sec.~\ref{sec:collisionChecking}. We additionally implement the adaptive risk allocation on Method 2.1, denoted by Method 2.1*. All other methods use equal allocation. We are interested in comparing two quantities: \emph{success rate} and \emph{computation time}. 
% The first is the success rate, defined as the rate at which the planner returns a solution within the given maximum planning duration. The second is the computation time, which indicates the computational complexity of the algorithms. 
Each scenario consisted of a 32x32 environment with 50 obstacles and 2, 3, 5, or 7 robots. Benchmarking was performed using 50 runs for each algorithm with a maximum planning time of 3 minutes. The results of the benchmarks for both systems are in Table \ref{tab:benchCCKCBS}. 

We see that Method 1 is consistently faster than the other methods for the linear system, although this advantage is less pronounced for the smallest system (2 robots), and largest system (7 robots) we studied. It appears to offer only limited benefit for the more complex unicycle system. We can additionally see that the adaptive risk allocation technique consistently outperforms the equal allocation, both in computation time and success rate.

\ml{remove this paragraph... add centralized to the table}
We additionally performed benchmarking on the centralized approach with the simple linear system, using collision checking Method 1. We allocated the full planning time for optimization, so computation time is not reported. The centralized approach allows optimization via the SST algorithm, which does result in improved sum of controls. However, it quickly runs into scalability problems, we were unable to scale beyond 3 robots, where the success rate was $8\%$.

\ml{fix this paragraph}
Finally, we note that CC-K-CBS was able to scale to 20 in a 32x32 environment containing 50 obstacles (with success rate $66\%$), and 25 robots in an empty environment (with success rate $xx\%$), with only collision checking Method 1.  All other methods timed out with more than 7 robots.

% \subsubsection{Planner Behavior}
\ml{show plan for 7 robots and simulations first...}
We present the nominal motion plans for 25 unicycle robots in Figure \ref{fig:unicycle_SampleTraj_big}, with the $p_\safe$ contours plotted as circles. We validated these nominal plans by determining that the contours do not intersect with each other or obstacles at any point. We additionally generated plans for 7 simple linear robots, and Monte Carlo sampled trajectories (shown in Figure \ref{fig:Simple2D_sampleTraj}) to verify that the total probability of collision was less than $1-p_\safe$.


\ml{integrate it with the environments description..}
To highlight how the scenario influences the planner behavior, consider the narrow corridor in Figure \ref{fig:Simple2D_sampleTraj_narrow}, with the simple 2D system, where the noise matrices were modified to be elliptical ($R^i=Q^i=diag(0.05^2,0.1^2)$). This accentuates the conservatism of Method 1: because the ellipse is aligned with the narrow corridor, the true probability of collision is not high, however the circular bound from Method 1 is unable to account for this. In this scenario, implementation of Method 1 in the planner does not find a plan, where implementation of all the other methods do. 

%We present sample plans generated by the K-CBS algorithm under both dynamics models with $p_\safe=0.90$. These plans were generated in a 32x32 environment containing 50 random obstacles. Figure \ref{fig:unicycle_SampleTraj_big} presents the nominal trajectories for 12 robots, with the $90\%$ confidence bound plotted as ellipses. We verified that these bounds do not simultaneously intersect at any point in the nominal trajectories, nor do they intersect with obstacles. We additionally verify the probability of collision over entire sampled trajectories for the simple 2D linear system using 500 MC samples of each robot's trajectory. The empirically obtained probability of collision was $3.7\%$ for the simple 2D system. Examples of the nominal plans and sampled trajectories for the simple 2D system are shown in Figure \ref{fig:Simple2D_sampleTraj}.



% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{figures/unicycle_SampleTraj.pdf}
%     \vspace{-2mm}
%     \caption{For the unicycle system, $95\%$ confidence bound plotted as ellipses, with the nominal trajectory over-plotted as a solid line for each of 7 agents.}
%     \label{fig:unicycle_sampleTraj}
%     \vspace{0mm}
% \end{figure}

% \begin{figure}
%     \centering
%     \begin{subfigure}{0.33\textwidth}
%     \includegraphics[angle=90,width=\textwidth]{figures/simpleLin_SampleTraj.pdf}
%     \vspace{-7mm}
%     \caption{}
%     \label{fig:Simple2D_sampleTraj}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.14\textwidth}
%     \includegraphics[width=\textwidth]{figures/simpleLin_SampleTraj_narrow.pdf}
%     \vspace{-7mm}
%     \caption{}
%     \label{fig:Simple2D_sampleTraj_narrow}
%     \end{subfigure}
%     \hfill

% \caption{(a) For the simple 2D system in a 32x32 environment: 100 MC sampled trajectories plotted as transparent lines, with the nominal trajectory over-plotted as a solid line. (b) Sample 6x2 narrow environment}
% \vspace{-3.5mm}
% \end{figure}



\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{figures/simpleLin_SampleTraj.pdf}
    \vspace{-2mm}
    \caption{For the simple 2D system in a 32x32 environment: 100 MC sampled trajectories plotted as transparent lines, with the nominal trajectory over-plotted as a solid line.}
    \label{fig:Simple2D_sampleTraj}
    \vspace{-5mm}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[angle=90,width=0.25\textwidth]{figures/simpleLin_SampleTraj_narrow.pdf}
    \vspace{-2mm}
    \caption{Sample 6x2 narrow environment}
    \label{fig:Simple2D_sampleTraj_narrow}
    \vspace{-5mm}
\end{figure}


==> sections/evaluation_IROSarxiv.tex <==

% We implemented CC-K-CBS with belief-SST as the low-lever planner in Open Motion Planning Library (OMPL), 
% The benchmarks were performed on AMD Ryzen 9 4.5GHz CPU and 64 GB of RAM.
We evaluate our algorithms in several benchmarks. We first focus on characterizing the robot-robot collision checking algorithms from Sec.~\ref{sec:collisionChecking} independent of the planning algorithm. This allows us to isolate the conservatism and computational complexity of the robot-robot collision checkers. We then analyze the full algorithms from Sec.~\ref{sec:method} with different collision checking methods.
Our implementation of CC-K-CBS uses belief-SST as the low-level planner in Open Motion Planning Library (OMPL) \cite{sucan2012the-open-motion-planning-library}. 
The benchmarks were performed on AMD 4.5 GHz CPU and 64 GB of RAM.
% this allows us to examine how the larger planning framework behaves as whole, and better evaluate the situations where one collision checker is advantageous over the other.

\begin{figure}
    \centering
    \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/conservatism.pdf}
    \vspace{-7mm}
    \caption{}
    \label{fig:conservatism}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.23\textwidth}
    \includegraphics[width=\textwidth]{figures/CompTime_combined.pdf}
    \vspace{-7mm}
    \caption{}
    \label{fig:compTime_combined}
    \end{subfigure}
    \hfill

\caption{(a) Plot of the conservatism $C_{z}$ for each method in each environment. (b) Box and whiskers plots of the log(computation time) for each method.}
\vspace{-3.5mm}
\end{figure}

We consider square-shaped robots of width 0.25 with two types of dynamics: 2D robotic system taken from~\cite{Bry2011_BeliefProp}:
\begin{equation*}
    x_{k+1}^i=x_k^i+u_k^i+w_k^i \qquad w_k^i \sim \mathcal{N}(0,0.1^2I),
\end{equation*}
% x_{k+1}^i=x_k^i+u_k^i+w_k^i$ with $w_k^i \sim \mathcal{N}(0,0.1^2I),
and 2nd-order unicycle:
\begin{equation*}
    \dot{\text{x}}^i= \text{v} \cos\theta, \quad \dot{\text{y}}^i= \text{v} \sin \theta, \quad \dot{\theta}=\omega, \quad \dot{\text{v}}=a,
\end{equation*}
% $\dot{\text{x}}^i= \text{v} \cos\theta,$ $\dot{\text{y}}^i= \text{v} \sin \theta$, $\dot{\theta}=\omega$, $\dot{\text{v}}=a$,
where $\omega$ and $a$ are control inputs. We use the feedback linearization 
scheme described in \cite{DeLuca2000_feedbackLin} 
to obtain a linear model, 
%with $x_k^i=[\text{x}_k^i,\dot{\text{x}}_k^i, \text{y}_k^i,\dot{\text{y}}_k^i]$ and noise $Q^i=0.1^2I$. 
which we convert to discrete time with additive noise. We assume both systems are fully observable with measurement model in \eqref{eq: measurement model} with $C^i=I$ and $R^i=0.1^2I$. 


% \subsection{Robot-Robot Collision Checker Benchmarking}
\textbf{Robot-Robot Collision Checker Benchmark: }
We characterize the robot-robot collision checking algorithms based on computation time and conservatism. Conservatism impacts the planners ability to find paths in more difficult, i.e. cluttered, situations. For a given set of beliefs for two robots, we define the conservatism of method $z$ as $C_{z} = R_{z} - R_{MC}$, where $R_{z}$ is the rejection rate obtained by method $z$, and $R_{MC}$ is the rejection rate obtained by a Monte Carlo evaluation of the probability of collision.

% from the \emph{true} probability of collision, $p_{true}^{ij}$. 

% If the true probability is know, the chance constraint can be exactly evaluated: $p_{true}^{ij}<1-p_\safe$. To evaluate conservatism, we randomly sampled $N_{MC}$ sets of two beliefs for each agent, $B_{s_{ij}}=\{\expBelief^i, \expBelief^j\}, s_{ij}=1,...,N_{MC}$, with $N_{MC}=10,000$. For each pair, we then computed the true probability of collision, and evaluated the chance constraint to obtain either valid or invalid, $\bar{v}^{s_{ij}}=1$ or $0$ respectively. The true validity rate can then be calculated as $\bar{V}_{true}=\sum_{s_{ij}=1}^{N_{MC}} \bar{v}^{s_{ij}}/N_{MC}$. For each pair, we then evaluate the chance constraint according to each of the proposed collision checking algorithm, $\bar{v}_{alg}^{s_{ij}}\in\{0,1\}$, yielding an associated algorithmic validity rate $\bar{V}_{alg}=\sum_{s_{ij}=1}^{N_{MC}} \bar{v}_{alg}^{s_{ij}}/N_{MC}$. Conservatism is defined as the difference between the true validity rate and the algorithmic validity rate: $C_{alg}=\bar{V}_{alg}-\bar{V}_{true}$. This indicates how often the algorithm rejects as invalid a sample that actually satisfies the chance constraint.


% \ml{all you're saying is that conservatism of method $z$ is defined as $C_{z} = R_{z} - R_{MC}$, where $R_{z}$ is the rejection rate obtained by method $z$, and $R_{MC}$ the rejection rate obtained by Monte Carlo evaluation of the probability of collision????}

% \ml{is this paragraph needed?}
% As stated earlier, the entire motivation for the proposed agent-agent collision checking algorithms is the difficulty of evaluating the true probability of collision. For the benchmarks performed here, we approximate the true probability of collision via MC sampling. For each pair of sampled beliefs, we further sampled 50,000 states. Each sampled state corresponds to a projection of the robots bodies in the workspace, where collision is indicated by the intersection of the two projections. To calculate the 'true' probability of collision, we found the proportion of the sampled states that resulted in collision.

We sampled 2D beliefs in two difference spaces, 5x5 and 10x10, with $p_\safe=0.95$. For Method 2.2 (the gridded cdf method), we chose 6 different grid discretizations, denoted by Method 2.2($d$). For each discretization, the maximum range of $\mathcal{P}_{whit}^{ij}$ over each axis, $D_w$, was divided equally, such that the discretization step size was $D_w/d$. Note that each of the proposed methods decreases in conservatism, shown in Fig.~\ref{fig:conservatism}, and increases in computation time, shown in Fig.~\ref{fig:compTime_combined}. The 5x5 space is the more `cluttered', with more beliefs in close proximity, which in turn results in higher collision probabilities. Note that the 5x5 space generally results in lower conservatism. This is because for the relatively high choice of $p_\safe$, a high proportion of the sampled beliefs truly violated the chance constraint, making it less conservative compared to a scenario where more beliefs are valid.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/PcollVSdist_Comp.pdf}
%     \vspace{-2mm}
%     \caption{Plot of the true probability of collision vs the euclidean distance between the means for each sampled belief pair}
%     \label{fig:PcollvsDist}
%     \vspace{0mm}
% \end{figure}



%%%%%%%%%%%%%%%%% SIDE BY SIDE TABLE
% \begin{table*}[]
% \caption{CC-K-CBS benchmarks for 2D system in Env8}
%     \centering
%     \scalebox{0.84}{
%     \begin{tabular}{|c|c||c|c|c|c|c|c||c|c|c|c|c|c|}
%          \hline
%          & & \multicolumn{6}{c||}{Simple Linear} & \multicolumn{6}{c|}{Unicycle}  \\ 
%         $N_A$ & Metric & M.1 & M.2.1 & M.2.1* & M.2.2(2) & M.2.2(5) & M.2.2(10)    \\ \hline 
%         \multirow{3}{*}{2} &  Succ. Rate &  1.00&   1.00 &   1.00 &   1.00 &   1.00 &   1.00 &  1.00&   1.00 &   1.00 &   1.00 &   1.00 &   1.00\\ 
%          &  Time (s) &    1.73 &   0.71 &   \textbf{0.56} &   0.87 &   1.19 &   0.75  & 0.03 &   0.03 &   0.05 &   0.04 &   0.04 &   0.06 \\ \hline 
%         \multirow{3}{*}{4} &  Succ. Rate &  0.00&   1.00 &   1.00 &   1.00 &   1.00 &   1.00  & 1.00&   1.00 &   1.00 &   1.00 &   1.00 &   1.00\\ 
%          &  Time (s) &     - &  11.86 &  41.92 &   \textbf{5.33} &   6.09 &  10.89  &    0.21 &   0.36 &   0.27 &   0.27 &   0.36 &   0.57   \\ \hline 
%         \multirow{3}{*}{6} &  Succ. Rate &  -&   0.00 &   0.20 &   1.00 &   1.00 &   1.00  &  0.00&   0.00 &   0.00 &   0.00 &   0.00 &   0.00 \\ 
%          &  Time (s) &     - &    - & 127.82 &   \textbf{5.53} &   8.61 &  16.43   &     NaN &    NaN &    NaN &    NaN &    NaN &    NaN  \\ \hline 
%         \multirow{3}{*}{8} &  Succ. Rate &  -&   - &   0.00 &   \textbf{0.98} &   0.94 &   0.90   &   1.00  &  0.00&   0.00 &   0.00 &   0.00 &   0.00  \\ 
%          &  Time (s) &    - &   - &   0.00 &  \textbf{18.56} &  29.77 &  61.79  &     NaN &    NaN &    NaN &    NaN &    NaN &    NaN   \\ \hline     
%     \end{tabular}
%     }
%     \label{tab:benchCCKCBS}
% \end{table*}



\begin{figure}[t]
    \centering
    \begin{subfigure}[b]{0.49\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/unicycle_SampleTraj_8x8.pdf}
         \caption{Env8}
         \label{fig:unicycle_SampleTraj_8x8}
     \end{subfigure}
    \begin{subfigure}[b]{0.49\columnwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/unicycle_SampleTraj_32x32obs.png}
         \caption{Env32Obs}
         \label{fig:unicycle_SampleTraj_32x32obs}
     \end{subfigure}
     \hfill
     \hspace{-2mm}
     \caption{(a) Sample plan for 4 robots with 2nd-order unicycle dynamics in Env8. Ellipses are $95\%$ probability contours. (b) Sample plan for 20 robots with 2nd-order unicycle dynamics in Env32Obs. Ellipses are $95\%$ probability contours.}
     \label{fig:envs}
\end{figure}

%%%%%%%%%%%%%%%%% OLD RESULTS TABLE (JUST LINEAR)

% \begin{table}[]
% \caption{CC-K-CBS benchmarks for Env8 (OLD RESULTS)}
%     \centering
%     \scalebox{0.84}{
%     \begin{tabular}{|c|c|c|c|c|c|c|c|}
%          \hline
%         $N_A$ & Metric & M.1 & M.2.1 & M.2.1* & M.2.2(2) & M.2.2(5) & M.2.2(10) \\ \hline 
%         \multirow{3}{*}{2} &  Succ. Rate &  1.00&   1.00 &   1.00 &   1.00 &   1.00 &   1.00\\ 
%          &  Time (s) &    1.73 &   0.71 &   \textbf{0.56} &   0.87 &   1.19 &   0.75 \\ \hline 
%         \multirow{3}{*}{4} &  Succ. Rate &  0.00&   1.00 &   1.00 &   1.00 &   1.00 &   1.00\\ 
%          &  Time (s) &     - &  11.86 &  41.92 &   \textbf{5.33} &   6.09 &  10.89 \\ \hline 
%         \multirow{3}{*}{6} &  Succ. Rate &  -&   0.00 &   0.20 &   1.00 &   1.00 &   1.00\\ 
%          &  Time (s) &     - &    - & 127.82 &   \textbf{5.53} &   8.61 &  16.43 \\ \hline 
%         \multirow{3}{*}{8} &  Succ. Rate &  -&   - &   0.00 &   \textbf{0.98} &   0.94 &   0.90\\ 
%          &  Time (s) &    - &   - &   0.00 &  \textbf{18.56} &  29.77 &  61.79 \\ \hline   
%     \end{tabular}
%     }
%     \label{tab:benchCCKCBS}
% \end{table}




%%%%%%%%%%%%%%%%% NEW RESULTS STACKED TABLE
\begin{table}[]
\caption{CC-K-CBS benchmarks for Env8}
    \centering
    \scalebox{0.84}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|}
         \hline
         \multicolumn{8}{|c|}{2D Linear} \\ \hline
        $N_A$ & Metric & M.1 & M.2.1 & M.2.1* & M.2.2(2) & M.2.2(5) & M.2.2(10) \\ \hline 
        \multirow{3}{*}{2} &  Succ. Rate &  1.00&   1.00 &   1.00 &   1.00 &   1.00 &   1.00\\ 
         &  Time (s) &    1.08 &   \textbf{0.68} &   1.04 &   1.11 &   0.69 &   0.74 \\ \hline 
        \multirow{3}{*}{4} &  Succ. Rate &  0.00&   1.00 &   1.00 &   1.00 &   1.00 &   1.00\\ 
         &  Time (s) &     - &  18.68 &  35.03 &   4.19 &   \textbf{3.97} &   7.61 \\ \hline 
        \multirow{3}{*}{6} &  Succ. Rate &  -&   0.00 &   0.12 &   1.00 &   1.00 &   1.00\\ 
         &  Time (s) &     - &    - &  66.68 &   \textbf{4.44} &   6.15 &  12.72 \\ \hline 
        \multirow{3}{*}{8} &  Succ. Rate &  -&   - &   0.00 &   1.00 &   1.00 &   0.86\\ 
         &  Time (s) &     - &    - &    - &  \textbf{15.38} &  26.54 &  59.08 \\ \hline  
         \multicolumn{8}{|c|}{Unicycle} \\ \hline
        \multirow{3}{*}{2} &  Succ. Rate &  1.00&   1.00 &   1.00 &   1.00 &   1.00 &   1.00\\ 
         &  Time (s) &    0.95 &   0.63 &   0.61 &   \textbf{0.37} &   0.57 &   0.83 \\ \hline 
        \multirow{3}{*}{4} &  Succ. Rate &  0.00&   0.96 &   1.00 &   1.00 &   1.00 &   1.00\\ 
         &  Time (s) &     - &  17.67 &   9.81 &   \textbf{2.59} &   2.86 &   5.24 \\ \hline 
        \multirow{3}{*}{6} &  Succ. Rate & -&   0.00 &   0.00 &   1.00 &   1.00 &   1.00\\ 
         &  Time (s) &     - &    - &    - &   \textbf{4.79} &   5.95 &  10.40 \\ \hline 
        \multirow{3}{*}{8} &  Succ. Rate &  -&   - &   - &   1.00 &   0.98 &   0.96\\ 
         &  Time (s) &     - &    - &    - &  \textbf{18.27} &  25.52 &  45.73 \\ \hline 
    \end{tabular}
    }
    \label{tab:benchCCKCBS}
\end{table}





% \subsection{Characterizing the MRMP Planners}
\textbf{Planners Benchmark: }
% We first compare benchmarks on the performance of the centralized and CC-K-CBS planners proposed in Sec.~\ref{sec:method}. We then present specific plans generated by the decentralized method, along with results from Monte Carlo (MC) simulations demonstrating the plans' validity. 
% \subsubsection{Planner Benchmarking}
We use benchmarking to evaluate the proposed planners under each of the collision-checking methods in Sec.~\ref{sec:collisionChecking}. We additionally implement the adaptive risk allocation on Method 2.1, denoted by M.2.1*. All other methods use equal allocation. 
% We are interested in comparing two quantities: \emph{success rate} and \emph{computation time}. 
% The first is the success rate, defined as the rate at which the planner returns a solution within the given maximum planning duration. The second is the computation time, which indicates the computational complexity of the algorithms. 
Benchmarking was performed using 50 runs for each algorithm with a maximum planning time of 3 minutes and $P_\safe = 0.9$. We examine 3 environments: a small 8x8 (Env8), large 32x32 with 50 random obstacles (Env32Obs), and large 32x32 without obstacles (Env32) shown in Figs.~\ref{fig:unicycle_SampleTraj_8x8}, \ref{fig:unicycle_SampleTraj_32x32obs}, and \ref{fig:unicycle_SampleTraj_big}, respectively.

%%%%%% BACKUP PARAGRAPH
\textit{Env8: } This small environment allows us to study how the different collision checking methods perform in a cluttered environment with the 2D system. The results are shown in Table~\ref{tab:benchCCKCBS}. Here the conservatism of the method strongly impacts the planners ability to find paths when more agents are introduced. All methods reliably find plans for 2 robots, however as the conservatism of the method increases, the success rate decreases when more agents are added. In this cluttered environment robot paths are necessarily close together, so more conservative methods are less likely to find valid paths.  Specifically, Method 1 performs poorly and Method 2.2 has the best performance.

% \textit{Env8: } This small environment allows us to study how the difference collision checking methods perform in a cluttered environment. The results are shown in Table~\ref{tab:benchCCKCBS}. Here the conservatism of the method strongly impacts the planners ability to find paths when more agents are introduced. All methods reliably find plans for 2 robots, however as the conservatism of the method increases, the success rate decreases when more agents are added. In this cluttered environment robot paths are necessarily close together, so more conservative methods are less likely to find valid paths.  Specifically, Method 1 performs poorly and Method 2.2 has the best performance.

\textit{Env32Obs: } The large environment is far less cluttered, allowing for far more agents and better insight into the scalability of the CC-K-CBS algorithm. The results for Env8 are based on the agent-obstacle collision checker from \cite{Luders2010_CC-RRT}. However, this is a very conservative collision checker, especially with a large number of obstacles.  CC-K-CBS with this method was unable to find paths in Env32Obs for even 2 robots. In the interest of scaling to larger numbers of robots, we made the very straightforward adaptation to Method 1 to check intersection of the bound $\mathcal{C}_{bound}^i$ with obstacles. 
As shown in Fig~\ref{fig:benchmark 30robots}, CC-K-CBS is able to scale to $20$ robots with $68\%$ success rate and runtime of $120.7\pm5.45$ seconds for the 2nd-order unicycle dynamics. A sample plan is shown in Fig.~\ref{fig:unicycle_SampleTraj_32x32obs}.  This illustrates that for large number of robots, Method 1 has the best performance because it is not affected by risk allocation, whereas the allocated risk gets much smaller as the number of robots increases for the other methods, making it difficult to find valid plans.

We also performed benchmarking on the centralized approach with the simpler 2D system in Env32Obs, using collision checking Method 1. 
% We allocated the full planning time for optimization, so computation time is not reported. The centralized approach allows optimization via the SST algorithm, which does result in improved sum of controls. However, it quickly runs into scalability problems, 
This algorithm was able to plan for 2 robots with $100\%$ success rate, but the success rate dropped to $8\%$ for 3 robots, illustrating the classical scalability issue with centralized approaches. 

\textit{Env32: } To further test the scalability of CC-K-CBS, we increased the number of agents in the large open environment Env32. 
As shown in Fig~\ref{fig:benchmark 30robots}, CC-K-CBS is able to to scale to $28$ 2nd-order unicycle robots with $56\%$ success rate and $129\pm4.97$ seconds computation time. 
A sample plan is shown in Fig.~\ref{fig:unicycle_SampleTraj_big}.  CC-K-CBS is also able to plan for 30 robots but at much lower success rate of $18\%$.

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/compareBench_32x32.pdf}
    % \vspace{-2mm}
    \caption{Benchmark results for CC-K-CBS on varying number of 2nd-oder unicycle robots. For \# robots $\leq 20$ we use Env32Obs, and for \# robots $\geq 22$ we use Env32.
    }
    \label{fig:benchmark 30robots}
    % \vspace{-5mm}
\end{figure}


% \subsubsection{Planner Behavior}
We validated the robustness of the motion plans using Monte Carlo simulation. We randomly selected motion plans, and with 500 simulations for each robot and observed no more than $2\%$ collision probability over the entire trajectory, illustrating the plans are indeed robust to uncertainty. 

%We present sample plans generated by the K-CBS algorithm under both dynamics models with $p_\safe=0.90$. These plans were generated in a 32x32 environment containing 50 random obstacles. Figure \ref{fig:unicycle_SampleTraj_big} presents the nominal trajectories for 12 robots, with the $90\%$ confidence bound plotted as ellipses. We verified that these bounds do not simultaneously intersect at any point in the nominal trajectories, nor do they intersect with obstacles. We additionally verify the probability of collision over entire sampled trajectories for the simple 2D linear system using 500 MC samples of each robot's trajectory. The empirically obtained probability of collision was $3.7\%$ for the simple 2D system. Examples of the nominal plans and sampled trajectories for the simple 2D system are shown in Figure \ref{fig:Simple2D_sampleTraj}.



% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{figures/unicycle_SampleTraj.pdf}
%     \vspace{-2mm}
%     \caption{For the unicycle system, $95\%$ confidence bound plotted as ellipses, with the nominal trajectory over-plotted as a solid line for each of 7 agents.}
%     \label{fig:unicycle_sampleTraj}
%     \vspace{0mm}
% \end{figure}

% \begin{figure}
%     \centering
%     \begin{subfigure}{0.33\textwidth}
%     \includegraphics[angle=90,width=\textwidth]{figures/simpleLin_SampleTraj.pdf}
%     \vspace{-7mm}
%     \caption{}
%     \label{fig:Simple2D_sampleTraj}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.14\textwidth}
%     \includegraphics[width=\textwidth]{figures/simpleLin_SampleTraj_narrow.pdf}
%     \vspace{-7mm}
%     \caption{}
%     \label{fig:Simple2D_sampleTraj_narrow}
%     \end{subfigure}
%     \hfill

% \caption{(a) For the simple 2D system in a 32x32 environment: 100 MC sampled trajectories plotted as transparent lines, with the nominal trajectory over-plotted as a solid line. (b) Sample 6x2 narrow environment}
% \vspace{-3.5mm}
% \end{figure}





==> sections/intro.tex <==

Robotic teams with diverse capabilities provide a powerful tool for efficiently accomplishing complex tasks. 
Applications extend from planetary exploration to automated warehouses and search and rescue missions.  However, planning for many robots is a challenging problem.
A major difficulty of \textit{multi-robot motion planning} (MRMP) lies in the size of the planning space, which grows exponentially with the number of robots. There
are also constraints posed by the robots' kinodynamics as well as robot-robot and robot-obstacle collisions that need to
be respected, which by itself is a difficult problem even for a
single robot. 
% A core challenge in \textit{multi-robot motion planning} (MRMP) is ensuring all robots avoid collision with each other and obstacles while accomplishing the assigned task. 
Additional complexities arise for realistic robots due to uncertainty in both motion and sensing, which the planner needs to account for in collision checking. 
In this work, we focus on the uncertain MRMP problem, and develop a scalable algorithm that guarantees collision avoidance and reaching goal with completeness properties.

Extensive work has considered MRMP problem in deterministic settings.
Proposed methods %is a well established research topic in robotics, and 
are either centralized (coupled)~\cite{Lavalle98rapidly-exploringrandom,wagner2015subdimensional,shome2020drrt,Kottinger:ICRA:2021,sucan2011sampling} or decentralized (decoupled)~\cite{gammell2014bit,tang2018complete,Le:ICAPS:2017,Le:RAL:2019}. %fall into two categories. %: centralized %(coupled) 
%and decentralized. %(decoupled). 
Centralized planners compose all robots' states together into a single meta-robot state, to which single-robot planning methods with completeness guarantees can then be applied. %Single robot planning techniques can then be readily applied to this meta-robot, which inherits their completeness properties. 
However, the exponential state increase makes centralized approaches scale poorly. Decentralized methods address this by planning for each robot individually and considering system collisions separately. These algorithms drastically cut computation time but often sacrifice completeness guarantees. For example, \cite{vandenBerg2005_prioritized} 
plans for one robot at a time, where each robot is constrained by the paths of all previously planned robots. While fast, this method is provably incomplete~\cite{lavalle2006planning}. % \at{citation?}. 
%  Other MRMP approaches use online distributed planning, e.g., \cite{Patwardhan2023_DistMRMP,AlonsoMora2018_CoopCollAvoid,Senbaslar2019_MultiRobotDistributed,VanParys2016_OnlineDistMultiVehicle}
%  \ml{are these for uncertain robots? This paragraph is for deterministic robots..}
%  ,
% %. These involve distributed planners, 
% where each robot plans over a short horizon to account for nearby robots and obstacles. %in the immediate vicinity. 
% These methods perform well in unknown environments where cooperation is not prioritized, but do not provide formal performance guarantees\jk{can we also say they do not provide correctness guarantees?}. %\at{I'm not really sure this paragraph is necessary...}
One recent contribution to scalable MRMP is Kinodynamic Conflict-Based Search (K-CBS), \cite{Kotting2022_KCBS}. K-CBS pairs a low-level kinodynamic motion planner for individual robots with a high-level tree search over the space of possible plans, which checks for robot-robot collisions and constructs the corresponding time dependent constraints to pass to the low-level motion planner. K-CBS offers users scalability and includes a merging technique to uphold probabilistic completeness properties of the low-level motion planner. Although a great step forward, none of these approaches are robust to state and measurement uncertainty, which are inherent to realistic robotic systems.  



\begin{figure}
    \centering
    \includegraphics[width=0.3\textwidth]{figures/unicycle_SampleTraj.png}
    \caption{Sample plans for 30 robots with 2nd-order unicycle dynamics under both motion and sensing uncertainties. Ellipses are $95\%$ safety contours. Star-centered circles are goal regions.}
    \label{fig:unicycle_SampleTraj_big}
    \vspace{-5mm}
\end{figure}

Motion planning under Gaussian uncertainty has largely been studied for single-robot systems. The most efficient of these are sampling-based planners, which are analogous to their deterministic counterparts, e.g., the feedback-based information roadmap \cite{Agha-Mohammadi2014_FIRM} %is an extension of probabilistic roadmaps (PRM), 
and rapidly-exploring random belief trees \cite{Bry2011_BeliefProp}. %are an extension of rapidly-exploring random trees (RRTs). 
%We adopt 
The belief-$\mathcal{A}$ framework introduced in \cite{Ho2022_GBT} provides a generic structure for adapting any sampling-based kinodynamic planner $\mathcal{A}$ to the belief space. It shows that fast planning is possible by using chance constraint formulation of collision avoidance.
Although these approaches can solve uncertain motion planning, they cannot solve uncertain MRMP out-of-the-box. 
% Wrapping this single agent planner in the K-CBS framework extends it to MRMP while maintaining %the planner's efficiency and performance guarantees. 

One approach to uncertain MRMP is to abstract the problem to a multi-agent Markov Decision Process (MMDP), which can be reduced to single-agent MDPs with a joint action space \cite{Boutilier1996_MMDP}. This relies on abstraction of the robot dynamics to a discretized transition probability matrix, which is difficult and scales poorly to many robots. Additionally, MMDPs solely account for uncertain dynamics, whereas measurement noise requires using a Partially-Observation MDP (POMDP), which can be very difficult to solve and also scales poorly.  Other uncertain MRMP approaches use online distributed planning, e.g., \cite{Patwardhan2023_DistMRMP,AlonsoMora2018_CoopCollAvoid,Senbaslar2019_MultiRobotDistributed,VanParys2016_OnlineDistMultiVehicle}, where each robot plans over a short horizon to account for nearby robots and obstacles. %in the immediate vicinity. 
These methods perform well in unknown environments. However, neither POMDP approaches nor online distributed methods provide any formal performance or completeness guarantees. %\at{I'm not really sure this paragraph is necessary...}

% On the other hand, single agent planners exist which do account for measurement noise and provide performance guarantees. 
 
% \nra{Zach Sunberg does, since he knows how to solve certain varieties quite efficiently, so not the best argument-rephrase/justify: *why* wouldn't you want this? doesn't provide any formal guarantees, or what?}. \nra{There is a disconnect in the argument here -- you go from talking about  MDPs/POMDPs for multiple robots to suddenly talking about single-robot planning techniques -- why?} 
%A broader variety of techniques exist for planning under uncertainty with a single robot \nra{...and so what? we can seek to adapt these to accommodate decentralized multi-robot planning under uncertainty? why are these worth looking at -- b/c in single-robot case they can provide guarantees under kinds of uncertainties we want to examine for multi-robot case? or something else?}. 

This work addresses this gap by presenting a scalable MRMP algorithm for robots operating with Gaussian state and measurement noise.
We combine %best aspects of K-CBS and belief-$\mathcal{A}$ to address MRMP under uncertainty: K-CBS enables 
the scalability of K-CBS with the fast belief-space planning of belief-$\mathcal{A}$ 
%enables fast belief space planning, and 
to solve MRMP for robots under Gaussian uncertainty. Our algorithm, Chance-Constrained K-CBS (CC-K-CBS), is probabilistically complete via the completeness inheritance properties of K-CBS and belief-$\mathcal{A}$~\cite{Kotting2022_KCBS,Ho2022_GBT}. 
% We present several new algorithms for probabilistic robot-robot collision checking. 

We present three main contributions: (i) three probabilistic robot-robot collision checking algorithms of varying conservatism and computational complexity; (ii) a scalable decentralized planner that uses novelties from (i) to solve MRMP for robots operating with Gaussian noise; 
%\nra{would be worth saying something a bit more technically insightful/appealing here -- why should reader keep on reading? are these new techniques that have not been developed previously?}\at{The techniques are kind simple, the novelty is in applying them in the multi-robot planning framework. Also, have not found many sources that directly benchmark computation and conservatism of collision checkers}; 
and (iii) case studies and benchmarks demonstrating the applicability of the larger MRMP framework, validity of our collision-checking methods, and comparisons between the algorithms. 
% Though the methods presented here are relatively simple, they have not been previously applied to multi-robot planning under uncertainty, and benchmarks evaluations for computation and conservatism have also not yet been established in this context. 



==> sections/method.tex <==


We now describe two algorithms for Chance-Constrained MRMP (CC-MRMP). We begin by formalizing the composed belief space for $N_A$ robots with models in \eqref{eq: dynamics model} and~\eqref{eq: measurement model}. We then propose a centralized approach to solving CC-MRMP by employing an existing single-robot belief-space planning algorithm called \emph{Belief-}$\mathcal{A}$ \cite{Ho2022_GBT}.
% which provides asymptotically optimal trajectories for systems described by Eqns.~\ref{eq: dynamics model} and~\ref{eq: measurement model}. 
To accommodate larger multi-robot systems, we introduce a decentralized algorithm called \emph{CC-K-CBS} which adapts the novel K-CBS algorithm to plan for systems with state and measurement uncertainty. We describe the empirical advantages and disadvantages of these methods in Sec.~\ref{sec:eval}.

\subsection{Centralized Chance-Constrained MRMP}
%Utilizing 
Centralized methods for uncertain MRMP require composing the system beliefs into a single \emph{meta-belief}, $\textbf{B}_k$, with a single dynamical constraint. We can then leverage the belief-$\mathcal{A}$ framework on this meta-belief.

Belief-$\mathcal{A}$ provides a framework for adapting any kinodynamic sampling-based planner $\mathcal{A}$ to efficiently plan in the Gaussian belief space \cite{Ho2022_GBT}, while providing guarantees on satisfying chance constraints on the probability of terminating in a goal region and the point-wise probability of collision. For brevity we only present an overview here, see \cite{Ho2022_GBT} for details. The algorithm builds a motion tree in Gaussian belief space the same way $\mathcal{A}$ does in the state space, e.g., if $\mathcal{A}$ is RRT, Belief-RRT extends the tree by sampling a random Gaussian belief, determining the closest node to that belief via the 2-Wasserstein distance, then extending that node using a computed nominal control input. The Gaussian belief is propagated 
% using the techniques derived in \cite{Bry2011_BeliefProp}. The propagated belief is 
and used for validity checking on the new node.  For collision checking, it adapts the method in \cite{Luders2010_CC-RRT}, which is based on linear constraint checking for static convex polytopic obstacles. 
% In our implementation we used this framework to adapt the Stable Sparse Rapidly Exploring Trees (SSTs)  algorithm, \cite{Li2016_SST}, to Belief-SST.

For centralized CC-MRMP, because all the robots are assumed to be independent, sampling and propagation of the meta-belief can be performed independently for each robot, and the meta-agent belief reconstructed from the individual robots' \emph{expected beliefs}, $\expBelief(x_k^i)$. These individual beliefs are obtained through \cite{Bry2011_BeliefProp}, which provides a method for predicting the belief over states for a linearizable and controllable system that uses a KF for estimation. This method forecasts the belief with a priori unknown measurements, yielding an expected belief defined as:
\begin{align*}
    \label{eq: expected belief}
    \expBelief(x_k^i) &= \mathbb{E}_Y[b(x_k^i \mid x_0^i, y_{0:k}^i)] 
    = \int_{y_{0:k}^i} \hspace{-3mm} b(x_k^i \mid x_0^i, y_{0:k}^i) pr(y_{0:k}^i)dy.
    % &= \mathcal{N}(\check{x}_k^i,\Sigma_k^i+\Lambda_k^i) = \mathcal{N}(\mu_k^i,\Gamma_k^i)
     % = \mathcal{N}(\mu_k^i,\Gamma_k^i),
\end{align*}
We use this expected belief for offline motion planning and evaluation of chance constraints in \eqref{eq:coll cc} and \eqref{eq: goal cc}. For a given initial belief $b(x_0^i)$ and nominal trajectory, $\check{X}^i$, the expected belief
$\expBelief(x_k^i) = \mathcal{N}(\check{x}_k^i,\Gamma_k^i)$, where $\Gamma_k^i = \Sigma_k^i+\Lambda_k^i$ can be recursively calculated as derived in \cite{Bry2011_BeliefProp}:
\begin{align}
    \Sigma_k^{i-} &= A\Sigma_{k-1}A^{iT} + Q^i, \quad \Sigma_k^i = \Sigma_k^{i-} - L_k^i C^i\Sigma_k^{i-}, \\
    \Lambda_k^i &= (A^i-B^iK^i)\Lambda_{k-1}^i(A^i-B^iK^i)^T + L_k^i C^i \Sigma_k^{i-},
\end{align}
where $\Sigma_k^i$ is the online KF uncertainty, and $\Lambda_k^i$ is covariance of the expected state estimates $\hat{x}_k^i$. Intuitively, this distribution can be thought of as the sum of the online estimation error and the uncertainty from the a priori unknown measurements made during execution. Given the expected beliefs for the agents, the meta-belief can be constructed such that $\textbf{B}_k=\mathcal{N}(\check{X}_k^{M}, \Gamma_k^M)$, where $\check{X}_k^{M}=(\check{x}_k^{iM}, ...,\check{x}_k^{N_A M})$, and $\Gamma_k^M$ is constructed as a bulk diagonal with elements $\Gamma_k^i, i=1,...,N_A$. 
Similarly, the validity checkers can be iterated for each robot, such that an entire meta-belief node is considered invalid if a single robot's belief is deemed invalid.

This centralized algorithm is the simplest of our two approaches, however it suffers from poor scalability with the number of agents, just as centralized deterministic planners do. To this end, we introduce a decentralized planner. 
% This formulation allows us to use any single-agent belief-space planner to solve uncertain MRMP. We denote this general algorithm as belief-$\mathcal{A}$, where $\mathcal{A}$ is any deterministic sampling-based tree planner. Originally introduced in \jk{cite}, belief-$\mathcal{A}$ works by sampling beliefs according to the Wasserstein distance metric, propagating the beliefs using Eqn.~\ref{eq: dynamics model} and~\ref{eq: measurement model} according to methods introduced in Bry/Roy \jk{cite}, and using off-the-shelf chance constrained agent-to-obstacle collision checkers to ensure safe solutions. Using belief-$\mathcal{A}$ for Uncertain MRMP adds an additional requirement of implementing an agent-to-agent collision checking procedure.  

\subsection{Decentralized Chance-Constrained K-CBS}
\begin{algorithm}[t]
\KwIn{$\W$, $\{x_0^i\}_{i=1}^{N_A}$, N, B, $p_{\safe}$}
\KwOut{Collision-free motion plans $\{(\check{U}^i, \check{X}^i)\}_{i=1}^{N_A}$}
$Q, n_0, \leftarrow \emptyset$;
$n_0$.plan $\leftarrow$ \underline{\textsc{getInitPlan}}$()$;$Q$.add($n_0$)\label{ln:rootNode}\;
$p_{safe}^A$,$p_{safe}^O \leftarrow$\underline{\textsc{allocSafety}}$(p_{\safe})$\;
\While{solution not found \label{ln:mainBegin}}
{
    $c \leftarrow$ $Q$.top()\label{ln:selectKCBS}\;
    \eIf{$c$.plan is empty \label{ln:retry}}
    {
        $Q$.pop(); \underline{\textsc{replan}}(N, $c$);
        % $\mathcal{C}_{\max} \leftarrow$
        % \If{shouldMerge($\mathcal{C}_{\max}$, B)\label{ln:mergeIf1}}
        % {
        %     \KwRet{mrg\&rstrt($\W$, $\{x_0^i\}_{i=1}^{N_A}$, N, B,$\mathcal{C}_{max}$)}
        % }
        $Q$.add($c$)\label{ln:retryAdd}\;
    }
    {
        K $\leftarrow$ \underline{\textsc{validatePlan}}($c$.plan, $p_{safe}^A$)\label{ln:validate}\;
        \uIf{K is empty\label{ln:isKempty}}
        {
            \KwRet{$c$.plan\label{ln:retPlan}}
        }
        \uElseIf{shouldMerge(K, B)\label{ln:shouldMerge}}
        {
            \KwRet{mrg\&rstrt($\W$, $\{x_0^i\}_{i=1}^{N_A}$, N, B,K)}
        }
        \Else
        {
            $Q$.pop()\label{ln:branchPop}\;
            \For{every robot $i$ in K\label{ln:branchForLoop}}
            {
                $c_{new}.\mathcal{C} \leftarrow$ $c.\mathcal{C} \: \cup$ \underline{\textsc{createCSTR}}(K, $i$)\;
                \underline{\textsc{replan}}(N, $c_{new}$); $Q$.add($c_{new}$)\label{ln:branchAdd}\; 
                %$\mathcal{C}_{\max} \leftarrow$ 
            }
        }
    }
    \label{ln:mainEnd}
}
\caption{Chance Constrained K-CBS}
\label{alg:G-KCBS}
\end{algorithm}
\setlength{\textfloatsep}{10pt}

Our decentralized CC-MRMP algorithm is based on Kinodynamic Conflict-Based Search (K-CBS)~\cite{Kotting2022_KCBS}. K-CBS consists of a high-level conflict-tree search and a low-level motion planner. At the high-level, K-CBS tracks a constraint-tree, in which each node represents a suggested plan, which might contain conflicts (i.e., collisions). At each iteration, K-CBS picks an unexplored node from the constraint-tree (CT), based on some heuristic, and identifies the conflicts in the node’s corresponding plan. Then, K-CBS tries to resolve the conflicts by creating child nodes as follows: if robot $i$ and $j$ collide for some finite time range $t\in[t_s,t_e]$ (denoted $\langle i,j,[t_s,t_e]\rangle$), then two child nodes are created, one with the constraint that $\mathcal{B}^i$ cannot intersect with $\mathcal{B}^j$ for all $t\in[t_s,t_e]$ and the other dually for robot $j$.
Then, in each child node, a low-level sampling-based planner attempts to replan a trajectory that satisfies the set of all constraints in that branch of the CT within $N>0$ iterations. This process repeats until a non-colliding plan is found. In the case where greater than $B>0$ conflicts arise, K-CBS includes a merge and restart procedure that recursively combines a subset of the robots. We refer the reader to~\cite{Kotting2022_KCBS} for details on the original K-CBS.
We now describe CC-K-CBS (Alg.~\ref{alg:G-KCBS}), which requires several adaptations of K-CBS (underlined in Alg.~\ref{alg:G-KCBS}).
% The pseudocode for (CC)-K-CBS is shown in Alg.~\ref{alg:G-KCBS}. We refer the reader to~\cite{Kotting2022_KCBS} for details on the original K-CBS. 

Firstly, note that in K-CBS, collision checking between robots and static obstacles are performed separately. The low-lever planner keeps track of workspace static obstacles, and the conflict tree accounts for robot-robot collisions at the high-level.  This separation is key for scalability, but it introduces a major challenge in chance-constrained planning for uncertain robots.  We expand on this further in Sec.~\ref{sec:collisionChecking}.
% We extended K-CBS Chance-Constrained K-CBS (CC-K-CBS) for CC-MRMP with three adaptations. 
% The procedures that require changes shown in red, blue, and violate fonts in Alg.~\ref{alg:G-KCBS}.
Secondly, since states are now beliefs, CC-K-CBS requires a Gaussian belief low-level motion planner.  We propose to use Belief-$\mathcal{A}$. As a result, the \textsc{replan} procedure returns a motion plan $(\check{U}^i, \check{X}^i)$ for robot $i$ while \textsc{getInitPlan} returns $(\check{U}^i, \check{X}^i)$ for all $i\in\{1, \ldots, N_A\}$. Thirdly, CC-K-CBS requires a definition of constraints; we introduce \emph{belief-constraints}. This simply replaces the deterministic shape with a non-deterministic belief. Thus, given a conflict $K=\langle i,j,[t_s,t_e]\rangle$, one constraint forces robot $i$ to satisfy the chance-constraint with $b(x_k^j)$ for all $t\in[t_s,t_e]$ and dually for robot $j$. This enables \textsc{createCSTR} in to define meaningful constraints during replanning with Belief-$\mathcal{A}$. 

Lastly, \textsc{validatePlan} requires an efficient way of validating the chance constraint while simulating prospective MRMP plans. We propose several techniques for this computation, each of which is described in detail in Sec.~\ref{sec:collisionChecking}. Every method requires comparison with the maximum allowable probability of collision $p_{coll} = 1-p_{\safe}$, the two-level structure of CC-K-CBS allows one to distribute $p_{coll}$ amongst the obstacles and robots. \textsc{allocSafety} can do this in a number of ways as explained in Sec.~\ref{sec:Risk Allocation}.  

% , such as normalizing by the percentage of obstacles and robots. Thus, $p_{coll}^A=1-p_{\safe}^A$ is the maximum allowable probability of unsafe behavior for robot-robot chance-constraint validation while $p_{coll}^O=1-p_{\safe}^O$ measures the same quantity for robot-obstacle chance constraint validations. Note that $p_{coll}^A+ p_{coll}^O=p_{coll}$.
\begin{theorem}[]
    \label{thm:completeness}
    If planner $\mathcal{A}$ is probabilistically complete, then so is CC-K-CBS.
\end{theorem}

\begin{proof}
Recall that if $\mathcal{A}$ is probabilistically complete, then so is Belief-$\mathcal{A}$~\cite{Ho2022_GBT}, which in turn implies K-CBS~\cite{Kotting2022_KCBS} is probabilistically complete. Therefore, if $\mathcal{A}$ is probabilistically complete, then so is CC-K-CBS.
\end{proof}



%These three new requirements present themselves inside the red, violet, and blue procedures of Alg.~\ref{alg:G-KCBS}, respectively. 


% \subsection{Belief Propagation}
% \label{sec:beliefProp}
% Work \cite{Bry2011_BeliefProp} provides a method for predicting the belief over states for a linearizable and controllable system that uses a KF for estimation. This method forecasts the belief with a priori unknown measurements, yielding an \emph{expected belief}, $\expBelief(x_k^i)$, defined as:
% \begin{align*}
%     \label{eq: expected belief}
%     \expBelief(x_k^i) &= \mathbb{E}_Y[b(x_k^i \mid x_0^i, y_{0:k}^i)] 
%     = \int_{y_{0:k}^i} \hspace{-3mm} b(x_k^i \mid x_0^i, y_{0:k}^i) pr(y_{0:k}^i)dy.
%     % &= \mathcal{N}(\check{x}_k^i,\Sigma_k^i+\Lambda_k^i) = \mathcal{N}(\mu_k^i,\Gamma_k^i)
%      % = \mathcal{N}(\mu_k^i,\Gamma_k^i),
% \end{align*}
% We use this expected belief for offline motion planning and evaluation of chance constraints \eqref{eq:coll cc} and \eqref{eq: goal cc}. For a given initial belief $b(x_0^i)$ and nominal trajectory, $\check{X}^i$, the expected belief
% $\expBelief(x_k^i) = \mathcal{N}(\check{x}_k^i,\Gamma_k^i)$, where $\Gamma_k^i = \Sigma_k^i+\Lambda_k^i$ can be recursively calculated as derived in \cite{Bry2011_BeliefProp}:
% \begin{align}
%     \Sigma_k^{i-} &= A\Sigma_{k-1}A^{iT} + Q^i, \quad \Sigma_k^i = \Sigma_k^{i-} - L_k^i C^i\Sigma_k^{i-}, \\
%     \Lambda_k^i &= (A^i-B^iK^i)\Lambda_{k-1}^i(A^i-B^iK^i)^T + L_k^i C^i \Sigma_k^{i-},
% \end{align}
% where $\Sigma_k^i$ is the online KF uncertainty, and $\Lambda_k^i$ is covariance of the expected state estimates $\hat{x}_k^i$. Intuitively, this distribution can be thought of as the sum of the online estimation error and the uncertainty from the a priori unknown measurements made during execution.


==> sections/problem.tex <==
% problem formulation

\subsection{Uncertain Multi-Robot System}
We consider $N_A$ uncertain robots in a shared workspace $\W \subset \reals^w$, $w\in\{2,3\}$ with a set of static obstacles $\W_O \subset \W$. Each robot $i \in \{1,\ldots, N_A\}$ has a rigid body $\B^i \subset \W$ and uncertain dynamics
\begin{equation}
\label{eq: dynamics model}
    x_{k+1}^i=A^ix_k^i + B^i u_k^i + w^i_k, \quad w_k^i \sim \N(0,Q^i), 
\end{equation}
where $x_k^i\in\X^i \subseteq\reals^{n_i}$ and $u_k^i\in\mathcal{U}^i \subseteq \reals^{p_i}$ are the state and controls, respectively, with the associated $A^i \in\reals^{n_i\times n_i}$ and $B^i \in\reals^{n_i\times p_i}$ matrices, and $w^i_k$ is the motion (process) noise sampled from a Gaussian distribution with zero mean and covariance $Q^i \in \reals^{n_i \times n_i}$. 

Note that state $x_k^i \in \X^i$ corresponds to the origin of the body frame of robot $\B^i$ w.r.t. to the global frame. The robot body $\B^i$ is defined as a set of points in its local frame. 
Since state $x_k^i$ includes configuration (position and orientation) as well as velocity terms, the body of the robot is well-defined w.r.t. global frame by projection of the state to either the configuration space (C-space) or workspace ($\W$).
 We define operator $\proj{\mathcal{S}}: \cup_{i=1}^{N_A} \X^i \to \mathcal{S}$ to be this projection of $x_k^i \in \X^i$ to its the lower dimensional space $\mathcal{S}\subset \X^i$, e.g., $\proj{\W}(x_k^i)\subset\W$ is the set of points ($\B^i$) that robot $i$ at state $x_k^i$ occupies in the workspace.

% \ml{do we have to assume measurement noise? it just makes it more complicated, no?}\at{Yes, but that's how the Gaussian belief trees are formulated, should keep it consistent with that?}
% \ml{GBT can be used with perfect measurement.... with process noise, we're still in the belief space}
Each robot $i \in \{1, \dots, N_A\}$ also has sensor (measurement) uncertainty described by
\begin{equation}
\label{eq: measurement model}
    y_k^i=C^ix_k^i + v^i_k, \quad v_k^i \sim\N(0,R^i), 
\end{equation}
where $y_k^i\in\Y^i \subseteq\reals^{m_i}$ is the sensor measurement, $C^i \in\reals^{m_i \times n_i}$ is the corresponding matrix, and $v_k^i$ is the measurement noise, sampled from Gaussian distribution with zero mean and covariance $R^i$. We additionally assume the system is both controllable and observable.


\subsection{Estimation, Control, and Motion Plan}
Each robot is equipped with a standard Kalman Filer (KF) and feedback controller.  The uncertainty of robot $i$ state, also known as the \textit{belief} of $x^i_k$ and denoted by $b(x^i_k)$,  is given by the KF as a Gaussian distribution at each time step $k$, i.e.,  
$$x^i_k \sim b(x_k^i)=\N(\hat{x}_k^i,\Sigma_k^i,)$$ 
where $\hat{x}_k^i \in \X^i$ is the state estimate (mean), and $\Sigma_k^i \in \reals^{n_i \times n_i}$ is the covariance matrix.  

We define \emph{motion plan} for robot $i$ to be a pair $(\check{U}^i,\check{X}^i)$ of nominal controls $\check{U}^i=(\check{u}_0^i, \check{u}_1^i, \ldots, \check{u}_{T-1}^i)$ and the corresponding trajectory of nominal states $\check{X}^i=(\check{x}_0^i, \check{x}_1^i, \ldots, \check{x}_T^i)$, where $\check{X}^i$ is obtained via propagation of the dynamics \eqref{eq: dynamics model} under $\check{U}^i$ in the absence of process noise.  Then, robot $i$ executes motion plan $(\check{U}^i, \check{X^i})$ by using a proportional stabilizing feedback controller
\begin{equation}
\label{eq:feedbackController}
    u_k^i = \check{u}_{k-1}^i - K(\hat{x}_k^i - \check{x}_k^i),
\end{equation}
where $K$ is the control gain.

% Each robot's initial state is Gaussian distributed with mean $\hat{x}_0^i$ and covariance $\Sigma_0^i$, i.e. $x_0^i\sim\N(\hat{x}_0^i,\Sigma_0^i)$.

\subsection{Probabilistic Collisions and Task Completion}
% \ml{Probabilistic Collision and Goal something?}

% \at{start with deterministic, then talk about probabilities, then constratin}
% \ml{let's not call it mission objectives... perhaps don't need to have a subsection here}\at{But we have to formally define the probability of collision before we can state the constraint in the problem formulation?}
% \ml{what I meant is that we don't need to have a subsection... it can be part of the main section.}



% We consider the task of navigating to a goal location while avoiding collision with obstacles and other agents. In a deterministic setting, where the state of the robot is known, this has been addressed by numerous sampling-based algorithms, \at{cite a few}. In each of these the projection of the body of the robot onto the workspace is always known, so checking for collision only involves checking known polyhedra for intersections. When the system dynamics are uncertain, as in \eqref{eq: dynamics model}, accomplishing the task becomes probabilistic. We can define the probability of reaching the goal, colliding with obstacles, and colliding with other agents in terms of the distributions across the agents' states.  

Each robot $i$ is assigned a goal region $\X_{G}^i\subset \X^i$  in its state space. 
The workspace contains $ |\W_O| = N_O$ static obstacles and $N_A$ robots (moving obstacles).  The motion planning task is to compute a plan for every robot to reach its goal and avoid collisions with all (static and moving) obstacles.  In a deterministic setting, these objectives (reaching goal and obstacle avoidance) are binary.  In a stochastic setting, they are probabilistic, which we define below.  

The probability that robot $i$ is in the goal region at time $k$ is given by 
\begin{equation}
    \label{eq:prob goal}
    P^{i_k}_G = P(x^i_k \in \X^i_G) = \int_{\X^i_G} b(x_k^i)(s) ds,
\end{equation}
where $b(x^i_k)(s)$ is the distribution $b(x^i_k)$ evaluated at state $s \in \X^i$.
For collision probability, we consider static and moving obstacles separately.  Let $\X^i_O \subseteq \X^i$ be the set of static obstacles in the robot $i$'s state space.  It is constructed from $\W_O$ (and the limits on the velocity terms).  Then, similar to probability of goal, the probability of collision of robot $i$ at time step $k$ with the static obstacles is
\begin{equation}
    \label{eq:prob collision}
    P^{i_k}_O = P(x^i_k \in \X^i_O) = \int_{\X^i_O} b(x_k^i)(s) ds.
\end{equation}
% \noindent

The probability of one robot colliding with another is more difficult to define because we must account for uncertainty in both robot bodies. To describe the collision states, it is best to consider the composed space of the two robots.  That is, for robot $i$ and $j$, $i \neq j$, define the composed state as $x^{ij} = (x^i, x^j) \in \X^i \times \X^j = \X^{ij}$.  The set of points that correspond to the two robots colliding is described by
\begin{multline*}
    \X^{ij}_\coll = \{x^{ij}=(x^i, x^j) \mid \proj{\W}(x^i) \cap \proj{\W}(x^i) \\
    \forall x^i \in \X^i, \; \forall x^j \in \X^j \}.
\end{multline*}
The probability of collision is then given by
\begin{align}
    P^{ij_k}_{\coll} &= P((x^i_k,x^j_k) \in \X^{ij}_\coll) = \int_{\X^{ij}_\coll} b(x_k^{ij})(s) ds \nonumber \\
    &= \int_{(s^i,s^j) \in \X^{ij}_\coll} \hspace{0 mm} b(x_k^{i})(s^i) b(x_k^{j})(s^j) ds^i ds^j,
    \label{eq:prob robot-robot collision}
\end{align}
where the equality in the second line is due to independence of the robots' uncertainties from each other.

In this work, we use a chance constraint to bound the safety (violating) probabilities.  That is, given a minimum probability of safety $p_\safe$, we want to ensure that probability of collision (with static and moving obstacles) at every time point is less than $1-p_\safe$, and the probability of ending in the goal is at least $p_\safe$.  

% While obstacles can be given in the state space $\X$, we assume these are linear constraints (such as velocity limits), that are easy to evaluate. Therefore, we focus our effort in this work on obstacles solely defined in workspace. A discrete trajectory of length $T^i$ agent $i$'s states is given by $X_{0:T}^i=(x_0^i, x_1^i, ..., x_T^i)$. We define the set of agent $i$ states for which the projection of its body intersects with an obstacle as $\X_{coll}^i=\{x^i \mid \proj{\W}(x_k^i))\cap\W_O\}$. 

% The probability of agent $i$ colliding with an obstacle at any time step $k$ in its trajectory is given by:
% \begin{equation}
%   P(\proj{\W}(x_k^i)) \cap \X_O) = \int_{\X_{coll}^i} p(x_k^i) dx,
% \end{equation}
% where $p(x_k^i)$ defines the probability distribution across agent $i$'s states at time step $k$. Note this probability describes the a priori distribution across states, and, while related, differs from the online estimate $b_k^i$ maintained by the KF. The method of obtaining this a priori distribution is discussed in Section \ref{sec:GBT}. The probability of agent $i$ terminating within its goal region is given by:
% \begin{equation}
%     P(x_T^i\in \X_{G}^i) = \int_{\X_{G}^i} p(x_T^i) dx
% \end{equation}


% The probability of one robot colliding with another is more difficult to define, because we must account for uncertainty in both robot bodies. 
% Consider a combined c-space representation for a pair of agents, $x_k^ij=(x_k^i, x_k^j)$. The probability at each point in this space (associated with a realization of paired states) is $p(x_k^i,x_k^j)$. Because we assumed the agents are independent we have $p(x_k^i,x_k^j)=p(x_k^i)p(x_k^j)$. We define the set of c-space points that result in collision as $\C_{coll}^{ij}=\{(x_k^i,x_k^j) \mid \proj{\W}(x_k^i) \cap \proj{\W}(x_k^j)\}$. Therefore, the probability of collision between agents $i$ and $j$ is given by:
% \begin{equation}
%     \label{eq:prob-coll}
%     P(\proj{\W}(X_k^i)) \cap \proj{\W}(X_k^j)) = \int_{\mathcal{C}_{coll}^{ij}} p(x_k^i)p(x_k^j) dx
% \end{equation}

% Note that the integration area $\C_{coll}^{ij}$ can be defined a priori, it is only the distribution $p(x_k^i,x_k^j)$ that changes with time. However, this area is still difficult to define, and very cumbersome to integrate. We address this in two ways. The fiest is the main contribution of this paper, and involves various methods to simplify this integral for efficient collision checking. The second is to consider only checking some constraint on the probability of collision, rather than calculating the actual probability of collision. Using chance constraints is a well established technique for planning with uncertain sysyems, \at{cite some things}. For each agent, we seek to constrain the point-wise probability of collision with obstacles an other agents, as well as constrain the probability of terminating in the desired goal region.


\subsection{Chance-Constrained MRMP Problem}
% \jk{Maybe put this in its own environment so we can reference ``Problem 1" throughout the paper.}
Given $N_A$ robots with uncertain dynamics in \eqref{eq: dynamics model}, noisy measurements in \eqref{eq: measurement model}, and controller \eqref{eq:feedbackController} in workspace $\W$ with static obstacles $\W_O$, 
a set of initial distributions $\{x_0^i = \N(\hat{x}_0^i,\Sigma^i_0)\}_{i=1}^{N_A}$, 
a set of goal regions $\{\X_G^i\}_{i=1}^{N_A}$, and a safety probability threshold $p_\safe$, for each robot $i \in \{1,\ldots,N_A\}$, compute a motion plan $(\check{U}^i, \check{X}^i) = ((\check{u}_0^i, \check{u}_1^i, \ldots, \check{u}_{T-1}^i), (\check{x}_0^i, \check{x}_1^i, \ldots, \check{x}_T^i))$ 
such that 
$\check{x}_0^i = \hat{x}_0^i$,
\begin{subequations}
    \begin{align}
        % P(\B^i \cap \X_O) \leq 1-p_\safe, \forall k=1,..,T, i=1,...,N_A \\
        % P(x_T^i\in \X_{goal}^i)\geq p_{\safe}, \forall i=1,...,N_A \\
        % P(\proj{\W}(X_{0:T}^i)) \cap \proj{\W}(X_{0:T}^j)) \leq 1-p_{\safe}, \\
        % \forall i\neq j, \forall t\in [0,max(T^i,T^j)]    
        \label{eq:coll cc}
        &P^{i_k}_O + \sum_{j=1, j \neq i}^{N_A} P^{ij_k}_{\coll} \leq 1-p_\safe && \forall k\in \{1,..,T\} \\
        \label{eq: goal cc}
        &P^{i_T}_G \geq p_{\safe} &&
    \end{align}    
\end{subequations}
where probability terms $P^{i_k}_O$, $P^{ij_k}_{\coll}$, and $P^{i_T}_G$ are given in \eqref{eq:prob collision}, \eqref{eq:prob robot-robot collision}, and \eqref{eq:prob goal}, respectively.

